AMED: Automatic Mixed-Precision Quantization for Edge Devices

Quantized neural networks are well known for reducing the latency, power consumption, and model size without significant harm to the performance. This makes them highly appropriate for systems with limited resources and low power capacity. Mixed-precision quantization offers better utilization of customized hardware that supports arithmetic operations at different bitwidths. Quantization methods either aim to minimize the compression loss given a desired reduction or optimize a dependent variable for a specified property of the model (such as FLOPs or model size); both make the performance inefficient when deployed on specific hardware, but more importantly, quantization methods assume that the loss manifold holds a global minimum for a quantized model that copes with the global minimum of the full precision counterpart. Challenging this assumption, we argue that the optimal minimum changes as the precision changes, and thus, it is better to look at quantization as a random process, placing the foundation for a different approach to quantize neural networks, which, during the training procedure, quantizes the model to a different precision, looks at the bit allocation as a Markov Decision Process, and then, finds an optimal bitwidth allocation for measuring specified behaviors on a specific device via direct signals from the particular hardware architecture. By doing so, we avoid the basic assumption that the loss behaves the same way for a quantized model. Automatic Mixed-Precision Quantization for Edge Devices (dubbed AMED) demonstrates its superiority over current state-of-the-art schemes in terms of the trade-off between neural network accuracy and hardware efficiency, backed by a comprehensive evaluation.

==> Definitions/journalnames.tex <==
%%Updated on 20 March 2024
%,% Website Name,%,%,% Website Name,%%,% Full Name,%%,% Short Name,%%,% DOI abbr,%%,% ISSN,% \continuouspages
%\DeclareOption{}{\gdef\@journal{}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{acoustics}{\gdef\@journal{acoustics}\gdef\@journalfull{Acoustics}\gdef\@journalshort{Acoustics}\gdef\@doiabbr{acoustics}\gdef\@ISSN{2624-599X}\gdef\@continuouspages{yes}}
\DeclareOption{actuators}{\gdef\@journal{actuators}\gdef\@journalfull{Actuators}\gdef\@journalshort{Actuators}\gdef\@doiabbr{act}\gdef\@ISSN{2076-0825}}
\DeclareOption{addictions}{\gdef\@journal{addictions}\gdef\@journalfull{Addictions}\gdef\@journalshort{Addictions}\gdef\@doiabbr{}\gdef\@ISSN{0006-0006}}
\DeclareOption{adhesives}{\gdef\@journal{adhesives}\gdef\@journalfull{Adhesives}\gdef\@journalshort{Adhesives}\gdef\@doiabbr{adhesives}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{admsci}{\gdef\@journal{admsci}\gdef\@journalfull{Administrative Sciences}\gdef\@journalshort{Adm. Sci.}\gdef\@doiabbr{admsci}\gdef\@ISSN{2076-3387}}
\DeclareOption{adolescents}{\gdef\@journal{adolescents}\gdef\@journalfull{Adolescents}\gdef\@journalshort{Adolescents}\gdef\@doiabbr{adolescents}\gdef\@ISSN{2673-7051}\gdef\@continuouspages{yes}}
\DeclareOption{aerobiology}{\gdef\@journal{aerobiology}\gdef\@journalfull{Aerobiology}\gdef\@journalshort{Aerobiology}\gdef\@doiabbr{aerobiology}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{aerospace}{\gdef\@journal{aerospace}\gdef\@journalfull{Aerospace}\gdef\@journalshort{Aerospace}\gdef\@doiabbr{aerospace}\gdef\@ISSN{2226-4310}}
\DeclareOption{agriculture}{\gdef\@journal{agriculture}\gdef\@journalfull{Agriculture}\gdef\@journalshort{Agriculture}\gdef\@doiabbr{agriculture}\gdef\@ISSN{2077-0472}}
\DeclareOption{agriengineering}{\gdef\@journal{agriengineering}\gdef\@journalfull{AgriEngineering}\gdef\@journalshort{AgriEngineering}\gdef\@doiabbr{agriengineering}\gdef\@ISSN{2624-7402}\gdef\@continuouspages{yes}}
\DeclareOption{agrochemicals}{\gdef\@journal{agrochemicals}\gdef\@journalfull{Agrochemicals}\gdef\@journalshort{Agrochemicals}\gdef\@doiabbr{agrochemicals}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{agronomy}{\gdef\@journal{agronomy}\gdef\@journalfull{Agronomy}\gdef\@journalshort{Agronomy}\gdef\@doiabbr{agronomy}\gdef\@ISSN{2073-4395}}
\DeclareOption{ai}{\gdef\@journal{ai}\gdef\@journalfull{AI}\gdef\@journalshort{AI}\gdef\@doiabbr{ai}\gdef\@ISSN{2673-2688}\gdef\@continuouspages{yes}}
\DeclareOption{air}{\gdef\@journal{air}\gdef\@journalfull{Air}\gdef\@journalshort{Air}\gdef\@doiabbr{air}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{algorithms}{\gdef\@journal{algorithms}\gdef\@journalfull{Algorithms}\gdef\@journalshort{Algorithms}\gdef\@doiabbr{a}\gdef\@ISSN{1999-4893}}
\DeclareOption{allergies}{\gdef\@journal{allergies}\gdef\@journalfull{Allergies}\gdef\@journalshort{Allergies}\gdef\@doiabbr{allergies}\gdef\@ISSN{2313-5786}}
\DeclareOption{alloys}{\gdef\@journal{alloys}\gdef\@journalfull{Alloys}\gdef\@journalshort{Alloys}\gdef\@doiabbr{alloys}\gdef\@ISSN{2674-063X}\gdef\@continuouspages{yes}}
\DeclareOption{amh}{\gdef\@journal{amh}\gdef\@journalfull{Acta Microbiologica Hellenica}\gdef\@journalshort{Acta Microbiol. Hell.}\gdef\@doiabbr{amh}\gdef\@ISSN{0438-9573}\gdef\@continuouspages{yes}}
\DeclareOption{analytica}{\gdef\@journal{analytica}\gdef\@journalfull{Analytica}\gdef\@journalshort{Analytica}\gdef\@doiabbr{analytica}\gdef\@ISSN{2673-4532}\gdef\@continuouspages{yes}}
\DeclareOption{analytics}{\gdef\@journal{analytics}\gdef\@journalfull{Analytics}\gdef\@journalshort{Analytics}\gdef\@doiabbr{analytics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{anatomia}{\gdef\@journal{anatomia}\gdef\@journalfull{Anatomia}\gdef\@journalshort{Anatomia}\gdef\@doiabbr{anatomia}\gdef\@ISSN{2813-0545}\gdef\@continuouspages{yes}}
\DeclareOption{anesthres}{\gdef\@journal{anesthres}\gdef\@journalfull{Anesthesia Research}\gdef\@journalshort{Anesth. Res.}\gdef\@doiabbr{anesthres}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{animals}{\gdef\@journal{animals}\gdef\@journalfull{Animals}\gdef\@journalshort{Animals}\gdef\@doiabbr{ani}\gdef\@ISSN{2076-2615}}
\DeclareOption{antibiotics}{\gdef\@journal{antibiotics}\gdef\@journalfull{Antibiotics}\gdef\@journalshort{Antibiotics}\gdef\@doiabbr{antibiotics}\gdef\@ISSN{2079-6382}}
\DeclareOption{antibodies}{\gdef\@journal{antibodies}\gdef\@journalfull{Antibodies}\gdef\@journalshort{Antibodies}\gdef\@doiabbr{antib}\gdef\@ISSN{2073-4468}}
\DeclareOption{antioxidants}{\gdef\@journal{antioxidants}\gdef\@journalfull{Antioxidants}\gdef\@journalshort{Antioxidants}\gdef\@doiabbr{antiox}\gdef\@ISSN{2076-3921}}
\DeclareOption{applbiosci}{\gdef\@journal{applbiosci}\gdef\@journalfull{Applied Biosciences}\gdef\@journalshort{Appl. Biosci.}\gdef\@doiabbr{applbiosci}\gdef\@ISSN{2813-0464}\gdef\@continuouspages{yes}}
\DeclareOption{appliedchem}{\gdef\@journal{appliedchem}\gdef\@journalfull{AppliedChem}\gdef\@journalshort{AppliedChem}\gdef\@doiabbr{appliedchem}\gdef\@ISSN{2673-9623}\gdef\@continuouspages{yes}}
\DeclareOption{appliedmath}{\gdef\@journal{appliedmath}\gdef\@journalfull{AppliedMath}\gdef\@journalshort{AppliedMath}\gdef\@doiabbr{appliedmath}\gdef\@ISSN{2673-9909}\gdef\@continuouspages{yes}}
\DeclareOption{applmech}{\gdef\@journal{applmech}\gdef\@journalfull{Applied Mechanics}\gdef\@journalshort{Appl. Mech.}\gdef\@doiabbr{applmech}\gdef\@ISSN{2673-3161}\gdef\@continuouspages{yes}}
\DeclareOption{applmicrobiol}{\gdef\@journal{applmicrobiol}\gdef\@journalfull{Applied Microbiology}\gdef\@journalshort{Appl. Microbiol.}\gdef\@doiabbr{applmicrobiol}\gdef\@ISSN{2673-8007}\gdef\@continuouspages{yes}}
\DeclareOption{applnano}{\gdef\@journal{applnano}\gdef\@journalfull{Applied Nano}\gdef\@journalshort{Appl. Nano}\gdef\@doiabbr{applnano}\gdef\@ISSN{2673-3501}\gdef\@continuouspages{yes}}
\DeclareOption{applsci}{\gdef\@journal{applsci}\gdef\@journalfull{Applied Sciences}\gdef\@journalshort{Appl. Sci.}\gdef\@doiabbr{app}\gdef\@ISSN{2076-3417}}
\DeclareOption{aquacj}{\gdef\@journal{aquacj}\gdef\@journalfull{Aquaculture Journal}\gdef\@journalshort{Aquac. J.}\gdef\@doiabbr{aquacj}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{architecture}{\gdef\@journal{architecture}\gdef\@journalfull{Architecture}\gdef\@journalshort{Architecture}\gdef\@doiabbr{architecture}\gdef\@ISSN{2673-8945}\gdef\@continuouspages{yes}}
\DeclareOption{arm}{\gdef\@journal{arm}\gdef\@journalfull{Advances in Respiratory Medicine}\gdef\@journalshort{Adv. Respir. Med.}\gdef\@doiabbr{arm}\gdef\@ISSN{2543-6031}\gdef\@continuouspages{yes}}
\DeclareOption{arthropoda}{\gdef\@journal{arthropoda}\gdef\@journalfull{Arthropoda}\gdef\@journalshort{Arthropoda}\gdef\@doiabbr{arthropoda}\gdef\@ISSN{2813-3323}\gdef\@continuouspages{yes}}
\DeclareOption{arts}{\gdef\@journal{arts}\gdef\@journalfull{Arts}\gdef\@journalshort{Arts}\gdef\@doiabbr{arts}\gdef\@ISSN{2076-0752}}
\DeclareOption{asc}{\gdef\@journal{asc}\gdef\@journalfull{Automatic Systems and Control}\gdef\@journalshort{Autom. Syst. Control}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{asi}{\gdef\@journal{asi}\gdef\@journalfull{Applied System Innovation}\gdef\@journalshort{Appl. Syst. Innov.}\gdef\@doiabbr{asi}\gdef\@ISSN{2571-5577}}
\DeclareOption{astronomy}{\gdef\@journal{astronomy}\gdef\@journalfull{Astronomy}\gdef\@journalshort{Astronomy}\gdef\@doiabbr{astronomy}\gdef\@ISSN{2674-0346}\gdef\@continuouspages{yes}}
\DeclareOption{atmosphere}{\gdef\@journal{atmosphere}\gdef\@journalfull{Atmosphere}\gdef\@journalshort{Atmosphere}\gdef\@doiabbr{atmos}\gdef\@ISSN{2073-4433}}
\DeclareOption{atoms}{\gdef\@journal{atoms}\gdef\@journalfull{Atoms}\gdef\@journalshort{Atoms}\gdef\@doiabbr{atoms}\gdef\@ISSN{2218-2004}}
\DeclareOption{audiolres}{\gdef\@journal{audiolres}\gdef\@journalfull{Audiology Research}\gdef\@journalshort{Audiol. Res.}\gdef\@doiabbr{audiolres}\gdef\@ISSN{2039-4349}\gdef\@continuouspages{yes}}
\DeclareOption{automation}{\gdef\@journal{automation}\gdef\@journalfull{Automation}\gdef\@journalshort{Automation}\gdef\@doiabbr{automation}\gdef\@ISSN{2673-4052}\gdef\@continuouspages{yes}}
\DeclareOption{axioms}{\gdef\@journal{axioms}\gdef\@journalfull{Axioms}\gdef\@journalshort{Axioms}\gdef\@doiabbr{axioms}\gdef\@ISSN{2075-1680}}
\DeclareOption{bacteria}{\gdef\@journal{bacteria}\gdef\@journalfull{Bacteria}\gdef\@journalshort{Bacteria}\gdef\@doiabbr{bacteria}\gdef\@ISSN{2674-1334}\gdef\@continuouspages{yes}}
\DeclareOption{batteries}{\gdef\@journal{batteries}\gdef\@journalfull{Batteries}\gdef\@journalshort{Batteries}\gdef\@doiabbr{batteries}\gdef\@ISSN{2313-0105}}
\DeclareOption{bdcc}{\gdef\@journal{bdcc}\gdef\@journalfull{Big Data and Cognitive Computing}\gdef\@journalshort{Big Data Cogn. Comput.}\gdef\@doiabbr{bdcc}\gdef\@ISSN{2504-2289}}
\DeclareOption{behavsci}{\gdef\@journal{behavsci}\gdef\@journalfull{Behavioral Sciences}\gdef\@journalshort{Behav. Sci.}\gdef\@doiabbr{bs}\gdef\@ISSN{2076-328X}}
\DeclareOption{beverages}{\gdef\@journal{beverages}\gdef\@journalfull{Beverages}\gdef\@journalshort{Beverages}\gdef\@doiabbr{beverages}\gdef\@ISSN{2306-5710}}
\DeclareOption{biochem}{\gdef\@journal{biochem}\gdef\@journalfull{BioChem}\gdef\@journalshort{BioChem}\gdef\@doiabbr{biochem}\gdef\@ISSN{2673-6411}\gdef\@continuouspages{yes}}
\DeclareOption{bioengineering}{\gdef\@journal{bioengineering}\gdef\@journalfull{Bioengineering}\gdef\@journalshort{Bioengineering}\gdef\@doiabbr{bioengineering}\gdef\@ISSN{2306-5354}}
\DeclareOption{biologics}{\gdef\@journal{biologics}\gdef\@journalfull{Biologics}\gdef\@journalshort{Biologics}\gdef\@doiabbr{biologics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biology}{\gdef\@journal{biology}\gdef\@journalfull{Biology}\gdef\@journalshort{Biology}\gdef\@doiabbr{biology}\gdef\@ISSN{2079-7737}}
\DeclareOption{biomass}{\gdef\@journal{biomass}\gdef\@journalfull{Biomass}\gdef\@journalshort{Biomass}\gdef\@doiabbr{biomass}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomechanics}{\gdef\@journal{biomechanics}\gdef\@journalfull{Biomechanics}\gdef\@journalshort{Biomechanics}\gdef\@doiabbr{biomechanics}\gdef\@ISSN{2673-7078}\gdef\@continuouspages{yes}}
\DeclareOption{biomed}{\gdef\@journal{biomed}\gdef\@journalfull{BioMed}\gdef\@journalshort{BioMed}\gdef\@doiabbr{biomed}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{biomedicines}{\gdef\@journal{biomedicines}\gdef\@journalfull{Biomedicines}\gdef\@journalshort{Biomedicines}\gdef\@doiabbr{biomedicines}\gdef\@ISSN{2227-9059}}
\DeclareOption{biomedinformatics}{\gdef\@journal{biomedinformatics}\gdef\@journalfull{BioMedInformatics}\gdef\@journalshort{BioMedInformatics}\gdef\@doiabbr{biomedinformatics}\gdef\@ISSN{2673-7426}\gdef\@continuouspages{yes}}
\DeclareOption{biomimetics}{\gdef\@journal{biomimetics}\gdef\@journalfull{Biomimetics}\gdef\@journalshort{Biomimetics}\gdef\@doiabbr{biomimetics}\gdef\@ISSN{2313-7673}}
\DeclareOption{biomolecules}{\gdef\@journal{biomolecules}\gdef\@journalfull{Biomolecules}\gdef\@journalshort{Biomolecules}\gdef\@doiabbr{biom}\gdef\@ISSN{2218-273X}}
\DeclareOption{biophysica}{\gdef\@journal{biophysica}\gdef\@journalfull{Biophysica}\gdef\@journalshort{Biophysica}\gdef\@doiabbr{biophysica}\gdef\@ISSN{2673-4125}\gdef\@continuouspages{yes}}
\DeclareOption{biosensors}{\gdef\@journal{biosensors}\gdef\@journalfull{Biosensors}\gdef\@journalshort{Biosensors}\gdef\@doiabbr{bios}\gdef\@ISSN{2079-6374}}
\DeclareOption{biotech}{\gdef\@journal{biotech}\gdef\@journalfull{BioTech}\gdef\@journalshort{BioTech}\gdef\@doiabbr{biotech}\gdef\@ISSN{2673-6284}}
\DeclareOption{birds}{\gdef\@journal{birds}\gdef\@journalfull{Birds}\gdef\@journalshort{Birds}\gdef\@doiabbr{birds}\gdef\@ISSN{2673-6004}\gdef\@continuouspages{yes}}
\DeclareOption{blockchains}{\gdef\@journal{blockchains}\gdef\@journalfull{Blockchains}\gdef\@journalshort{Blockchains}\gdef\@doiabbr{blockchains}\gdef\@ISSN{2813-5288}\gdef\@continuouspages{yes}}
\DeclareOption{bloods}{\gdef\@journal{bloods}\gdef\@journalfull{Bloods}\gdef\@journalshort{Bloods}\gdef\@doiabbr{bloods}\gdef\@ISSN{2673-415X}}
\DeclareOption{blsf}{\gdef\@journal{blsf}\gdef\@journalfull{Biology and Life Sciences Forum}\gdef\@journalshort{Biol. Life Sci. Forum}\gdef\@doiabbr{blsf	}\gdef\@ISSN{2673-9976}}
\DeclareOption{brainsci}{\gdef\@journal{brainsci}\gdef\@journalfull{Brain Sciences}\gdef\@journalshort{Brain Sci.}\gdef\@doiabbr{brainsci}\gdef\@ISSN{2076-3425}}
\DeclareOption{breath}{\gdef\@journal{breath}\gdef\@journalfull{Breath}\gdef\@journalshort{Breath}\gdef\@doiabbr{breath}\gdef\@ISSN{}}
\DeclareOption{buildings}{\gdef\@journal{buildings}\gdef\@journalfull{Buildings}\gdef\@journalshort{Buildings}\gdef\@doiabbr{buildings}\gdef\@ISSN{2075-5309}}
\DeclareOption{businesses}{\gdef\@journal{businesses}\gdef\@journalfull{Businesses}\gdef\@journalshort{Businesses}\gdef\@doiabbr{businesses}\gdef\@ISSN{2673-7116}\gdef\@continuouspages{yes}}
\DeclareOption{cancers}{\gdef\@journal{cancers}\gdef\@journalfull{Cancers}\gdef\@journalshort{Cancers}\gdef\@doiabbr{cancers}\gdef\@ISSN{2072-6694}}
\DeclareOption{carbon}{\gdef\@journal{carbon}\gdef\@journalfull{C}\gdef\@journalshort{C}\gdef\@doiabbr{c}\gdef\@ISSN{2311-5629}}
\DeclareOption{cardiogenetics}{\gdef\@journal{cardiogenetics}\gdef\@journalfull{Cardiogenetics}\gdef\@journalshort{Cardiogenetics}\gdef\@doiabbr{cardiogenetics}\gdef\@ISSN{2035-8148}\gdef\@continuouspages{yes}}
\DeclareOption{catalysts}{\gdef\@journal{catalysts}\gdef\@journalfull{Catalysts}\gdef\@journalshort{Catalysts}\gdef\@doiabbr{catal}\gdef\@ISSN{2073-4344}}
\DeclareOption{cells}{\gdef\@journal{cells}\gdef\@journalfull{Cells}\gdef\@journalshort{Cells}\gdef\@doiabbr{cells}\gdef\@ISSN{2073-4409}}
\DeclareOption{ceramics}{\gdef\@journal{ceramics}\gdef\@journalfull{Ceramics}\gdef\@journalshort{Ceramics}\gdef\@doiabbr{ceramics}\gdef\@ISSN{2571-6131}\gdef\@continuouspages{yes}}
\DeclareOption{challenges}{\gdef\@journal{challenges}\gdef\@journalfull{Challenges}\gdef\@journalshort{Challenges}\gdef\@doiabbr{challe}\gdef\@ISSN{2078-1547}}
\DeclareOption{chemengineering}{\gdef\@journal{chemengineering}\gdef\@journalfull{ChemEngineering}\gdef\@journalshort{ChemEngineering}\gdef\@doiabbr{chemengineering}\gdef\@ISSN{2305-7084}}
\DeclareOption{chemistry}{\gdef\@journal{chemistry}\gdef\@journalfull{Chemistry}\gdef\@journalshort{Chemistry}\gdef\@doiabbr{chemistry}\gdef\@ISSN{2624-8549}\gdef\@continuouspages{yes}}
\DeclareOption{chemosensors}{\gdef\@journal{chemosensors}\gdef\@journalfull{Chemosensors}\gdef\@journalshort{Chemosensors}\gdef\@doiabbr{chemosensors}\gdef\@ISSN{2227-9040}}
\DeclareOption{chemproc}{\gdef\@journal{chemproc}\gdef\@journalfull{Chemistry Proceedings}\gdef\@journalshort{Chem. Proc.}\gdef\@doiabbr{chemproc}\gdef\@ISSN{2673-4583}}
\DeclareOption{children}{\gdef\@journal{children}\gdef\@journalfull{Children}\gdef\@journalshort{Children}\gdef\@doiabbr{children}\gdef\@ISSN{2227-9067}}
\DeclareOption{chips}{\gdef\@journal{chips}\gdef\@journalfull{Chips}\gdef\@journalshort{Chips}\gdef\@doiabbr{chips}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{cimb}{\gdef\@journal{cimb}\gdef\@journalfull{Current Issues in Molecular Biology}\gdef\@journalshort{Curr. Issues Mol. Biol.}\gdef\@doiabbr{cimb}\gdef\@ISSN{1467-3045}\gdef\@continuouspages{yes}}
\DeclareOption{civileng}{\gdef\@journal{civileng}\gdef\@journalfull{CivilEng}\gdef\@journalshort{CivilEng}\gdef\@doiabbr{civileng}\gdef\@ISSN{2673-4109}\gdef\@continuouspages{yes}}
\DeclareOption{cleantechnol}{\gdef\@journal{cleantechnol}\gdef\@journalfull{Clean Technologies}\gdef\@journalshort{Clean Technol.}\gdef\@doiabbr{cleantechnol}\gdef\@ISSN{2571-8797}\gdef\@continuouspages{yes}}
\DeclareOption{climate}{\gdef\@journal{climate}\gdef\@journalfull{Climate}\gdef\@journalshort{Climate}\gdef\@doiabbr{cli}\gdef\@ISSN{2225-1154}}
\DeclareOption{clinpract}{\gdef\@journal{clinpract}\gdef\@journalfull{Clinics and Practice}\gdef\@journalshort{Clin. Pract.}\gdef\@doiabbr{clinpract}\gdef\@ISSN{2039-7283}\gdef\@continuouspages{yes}}
\DeclareOption{clockssleep}{\gdef\@journal{clockssleep}\gdef\@journalfull{Clocks \& Sleep}\gdef\@journalshort{Clocks\&Sleep}\gdef\@doiabbr{clockssleep}\gdef\@ISSN{2624-5175}\gdef\@continuouspages{yes}}
\DeclareOption{cmd}{\gdef\@journal{cmd}\gdef\@journalfull{Corrosion and Materials Degradation}\gdef\@journalshort{Corros. Mater. Degrad.}\gdef\@doiabbr{cmd}\gdef\@ISSN{2624-5558}\gdef\@continuouspages{yes}}
\DeclareOption{coasts}{\gdef\@journal{coasts}\gdef\@journalfull{Coasts}\gdef\@journalshort{Coasts}\gdef\@doiabbr{coasts}\gdef\@ISSN{2673-964X}\gdef\@continuouspages{yes}}
\DeclareOption{coatings}{\gdef\@journal{coatings}\gdef\@journalfull{Coatings}\gdef\@journalshort{Coatings}\gdef\@doiabbr{coatings}\gdef\@ISSN{2079-6412}}
\DeclareOption{colloids}{\gdef\@journal{colloids}\gdef\@journalfull{Colloids and Interfaces}\gdef\@journalshort{Colloids Interfaces}\gdef\@doiabbr{colloids}\gdef\@ISSN{2504-5377}}
\DeclareOption{colorants}{\gdef\@journal{colorants}\gdef\@journalfull{Colorants}\gdef\@journalshort{Colorants}\gdef\@doiabbr{colorants}\gdef\@ISSN{2079-6447}\gdef\@continuouspages{yes}}
\DeclareOption{commodities}{\gdef\@journal{commodities}\gdef\@journalfull{Commodities}\gdef\@journalshort{Commodities}\gdef\@doiabbr{commodities}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{compounds}{\gdef\@journal{compounds}\gdef\@journalfull{Compounds}\gdef\@journalshort{Compounds}\gdef\@doiabbr{compounds}\gdef\@ISSN{2673-6918}\gdef\@continuouspages{yes}}
\DeclareOption{computation}{\gdef\@journal{computation}\gdef\@journalfull{Computation}\gdef\@journalshort{Computation}\gdef\@doiabbr{computation}\gdef\@ISSN{2079-3197}}
\DeclareOption{computers}{\gdef\@journal{computers}\gdef\@journalfull{Computers}\gdef\@journalshort{Computers}\gdef\@doiabbr{computers}\gdef\@ISSN{2073-431X}}
\DeclareOption{condensedmatter}{\gdef\@journal{condensedmatter}\gdef\@journalfull{Condensed Matter}\gdef\@journalshort{Condens. Matter}\gdef\@doiabbr{condmat}\gdef\@ISSN{2410-3896}}
\DeclareOption{conservation}{\gdef\@journal{conservation}\gdef\@journalfull{Conservation}\gdef\@journalshort{Conservation}\gdef\@doiabbr{conservation}\gdef\@ISSN{2673-7159}\gdef\@continuouspages{yes}}
\DeclareOption{constrmater}{\gdef\@journal{constrmater}\gdef\@journalfull{Construction Materials}\gdef\@journalshort{Constr. Mater.}\gdef\@doiabbr{constrmater}\gdef\@ISSN{2673-7108}\gdef\@continuouspages{yes}}
\DeclareOption{cosmetics}{\gdef\@journal{cosmetics}\gdef\@journalfull{Cosmetics}\gdef\@journalshort{Cosmetics}\gdef\@doiabbr{cosmetics}\gdef\@ISSN{2079-9284}}
\DeclareOption{covid}{\gdef\@journal{covid}\gdef\@journalfull{COVID}\gdef\@journalshort{COVID}\gdef\@doiabbr{covid}\gdef\@ISSN{2673-8112}\gdef\@continuouspages{yes}}
\DeclareOption{crops}{\gdef\@journal{crops}\gdef\@journalfull{Crops}\gdef\@journalshort{Crops}\gdef\@doiabbr{crops}\gdef\@ISSN{2673-7655}\gdef\@continuouspages{yes}}
\DeclareOption{cryo}{\gdef\@journal{cryo}\gdef\@journalfull{Cryo}\gdef\@journalshort{Cryo}\gdef\@doiabbr{cryo}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{cryptography}{\gdef\@journal{cryptography}\gdef\@journalfull{Cryptography}\gdef\@journalshort{Cryptography}\gdef\@doiabbr{cryptography}\gdef\@ISSN{2410-387X}}
\DeclareOption{crystals}{\gdef\@journal{crystals}\gdef\@journalfull{Crystals}\gdef\@journalshort{Crystals}\gdef\@doiabbr{cryst}\gdef\@ISSN{2073-4352}}
\DeclareOption{csmf}{\gdef\@journal{csmf}\gdef\@journalfull{Computer Sciences \& Mathematics Forum}\gdef\@journalshort{Comput. Sci. Math. Forum}\gdef\@doiabbr{csmf}\gdef\@ISSN{2813-0324}}
\DeclareOption{ctn}{\gdef\@journal{ctn}\gdef\@journalfull{Clinical and Translational Neuroscience}\gdef\@journalshort{Clin. Transl. Neurosci.}\gdef\@doiabbr{ctn}\gdef\@ISSN{2514-183X}}
\DeclareOption{curroncol}{\gdef\@journal{curroncol}\gdef\@journalfull{Current Oncology}\gdef\@journalshort{Curr. Oncol.}\gdef\@doiabbr{curroncol}\gdef\@ISSN{1718-7729}\gdef\@continuouspages{yes}}
\DeclareOption{cyber}{\gdef\@journal{cyber}\gdef\@journalfull{Cyber}\gdef\@journalshort{Cyber}\gdef\@doiabbr{cyber}\gdef\@ISSN{2624-800X}}
\DeclareOption{dairy}{\gdef\@journal{dairy}\gdef\@journalfull{Dairy}\gdef\@journalshort{Dairy}\gdef\@doiabbr{dairy}\gdef\@ISSN{2624-862X}\gdef\@continuouspages{yes}}
\DeclareOption{data}{\gdef\@journal{data}\gdef\@journalfull{Data}\gdef\@journalshort{Data}\gdef\@doiabbr{data}\gdef\@ISSN{2306-5729}}
\DeclareOption{ddc}{\gdef\@journal{ddc}\gdef\@journalfull{Drugs and Drug Candidates}\gdef\@journalshort{Drugs Drug Candidates}\gdef\@doiabbr{ddc}\gdef\@ISSN{2813-2998}\gdef\@continuouspages{yes}}
\DeclareOption{dentistry}{\gdef\@journal{dentistry}\gdef\@journalfull{Dentistry Journal}\gdef\@journalshort{Dent. J.}\gdef\@doiabbr{dj}\gdef\@ISSN{2304-6767}}
\DeclareOption{dermato}{\gdef\@journal{dermato}\gdef\@journalfull{Dermato}\gdef\@journalshort{Dermato}\gdef\@doiabbr{dermato}\gdef\@ISSN{2673-6179}\gdef\@continuouspages{yes}}
\DeclareOption{dermatopathology}{\gdef\@journal{dermatopathology}\gdef\@journalfull{Dermatopathology}\gdef\@journalshort{Dermatopathology}\gdef\@doiabbr{dermatopathology}\gdef\@ISSN{2296-3529}\gdef\@continuouspages{yes}}
\DeclareOption{designs}{\gdef\@journal{designs}\gdef\@journalfull{Designs}\gdef\@journalshort{Designs}\gdef\@doiabbr{designs}\gdef\@ISSN{2411-9660}}
\DeclareOption{devices}{\gdef\@journal{devices}\gdef\@journalfull{Devices}\gdef\@journalshort{Devices}\gdef\@doiabbr{devices}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{diabetology}{\gdef\@journal{diabetology}\gdef\@journalfull{Diabetology}\gdef\@journalshort{Diabetology}\gdef\@doiabbr{diabetology}\gdef\@ISSN{2673-4540}\gdef\@continuouspages{yes}}
\DeclareOption{diagnostics}{\gdef\@journal{diagnostics}\gdef\@journalfull{Diagnostics}\gdef\@journalshort{Diagnostics}\gdef\@doiabbr{diagnostics}\gdef\@ISSN{2075-4418}}
\DeclareOption{dietetics}{\gdef\@journal{dietetics}\gdef\@journalfull{Dietetics}\gdef\@journalshort{Dietetics}\gdef\@doiabbr{dietetics}\gdef\@ISSN{2674-0311}\gdef\@continuouspages{yes}}
\DeclareOption{digital}{\gdef\@journal{digital}\gdef\@journalfull{Digital}\gdef\@journalshort{Digital}\gdef\@doiabbr{digital}\gdef\@ISSN{2673-6470}\gdef\@continuouspages{yes}}
\DeclareOption{disabilities}{\gdef\@journal{disabilities}\gdef\@journalfull{Disabilities}\gdef\@journalshort{Disabilities}\gdef\@doiabbr{disabilities}\gdef\@ISSN{2673-7272}\gdef\@continuouspages{yes}}
\DeclareOption{diseases}{\gdef\@journal{diseases}\gdef\@journalfull{Diseases}\gdef\@journalshort{Diseases}\gdef\@doiabbr{diseases}\gdef\@ISSN{2079-9721}}
\DeclareOption{diversity}{\gdef\@journal{diversity}\gdef\@journalfull{Diversity}\gdef\@journalshort{Diversity}\gdef\@doiabbr{d}\gdef\@ISSN{1424-2818}}
\DeclareOption{dna}{\gdef\@journal{dna}\gdef\@journalfull{DNA}\gdef\@journalshort{DNA}\gdef\@doiabbr{dna}\gdef\@ISSN{2673-8856}\gdef\@continuouspages{yes}}
\DeclareOption{drones}{\gdef\@journal{drones}\gdef\@journalfull{Drones}\gdef\@journalshort{Drones}\gdef\@doiabbr{drones}\gdef\@ISSN{2504-446X}}
\DeclareOption{dynamics}{\gdef\@journal{dynamics}\gdef\@journalfull{Dynamics}\gdef\@journalshort{Dynamics}\gdef\@doiabbr{dynamics}\gdef\@ISSN{2673-8716}\gdef\@continuouspages{yes}}
\DeclareOption{earth}{\gdef\@journal{earth}\gdef\@journalfull{Earth}\gdef\@journalshort{Earth}\gdef\@doiabbr{earth}\gdef\@ISSN{2673-4834}\gdef\@continuouspages{yes}}
\DeclareOption{ebj}{\gdef\@journal{ebj}\gdef\@journalfull{European Burn Journal}\gdef\@journalshort{Eur. Burn J.}\gdef\@doiabbr{ebj}\gdef\@ISSN{2673-1991}\gdef\@continuouspages{yes}}
\DeclareOption{ecm}{\gdef\@journal{ecm}\gdef\@journalfull{Emergency Care and Medicine}\gdef\@journalshort{Emerg. Care Med.}\gdef\@doiabbr{ecm}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{ecologies}{\gdef\@journal{ecologies}\gdef\@journalfull{Ecologies}\gdef\@journalshort{Ecologies}\gdef\@doiabbr{ecologies}\gdef\@ISSN{2673-4133}\gdef\@continuouspages{yes}}
\DeclareOption{econometrics}{\gdef\@journal{econometrics}\gdef\@journalfull{Econometrics}\gdef\@journalshort{Econometrics}\gdef\@doiabbr{econometrics}\gdef\@ISSN{2225-1146}}
\DeclareOption{economies}{\gdef\@journal{economies}\gdef\@journalfull{Economies}\gdef\@journalshort{Economies}\gdef\@doiabbr{economies}\gdef\@ISSN{2227-7099}}
\DeclareOption{education}{\gdef\@journal{education}\gdef\@journalfull{Education Sciences}\gdef\@journalshort{Educ. Sci.}\gdef\@doiabbr{educsci}\gdef\@ISSN{2227-7102}}
\DeclareOption{ejihpe}{\gdef\@journal{ejihpe}\gdef\@journalfull{European Journal of Investigation in Health, Psychology and Education}\gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}\gdef\@doiabbr{ejihpe}\gdef\@ISSN{2254-9625}\gdef\@continuouspages{yes}}
\DeclareOption{electricity}{\gdef\@journal{electricity}\gdef\@journalfull{Electricity}\gdef\@journalshort{Electricity}\gdef\@doiabbr{electricity}\gdef\@ISSN{2673-4826}\gdef\@continuouspages{yes}}
\DeclareOption{electrochem}{\gdef\@journal{electrochem}\gdef\@journalfull{Electrochem}\gdef\@journalshort{Electrochem}\gdef\@doiabbr{electrochem}\gdef\@ISSN{2673-3293}\gdef\@continuouspages{yes}}
\DeclareOption{electronicmat}{\gdef\@journal{electronicmat}\gdef\@journalfull{Electronic Materials}\gdef\@journalshort{Electron. Mater.}\gdef\@doiabbr{electronicmat}\gdef\@ISSN{2673-3978}\gdef\@continuouspages{yes}}
\DeclareOption{electronics}{\gdef\@journal{electronics}\gdef\@journalfull{Electronics}\gdef\@journalshort{Electronics}\gdef\@doiabbr{electronics}\gdef\@ISSN{2079-9292}}
\DeclareOption{encyclopedia}{\gdef\@journal{encyclopedia}\gdef\@journalfull{Encyclopedia}\gdef\@journalshort{Encyclopedia}\gdef\@doiabbr{encyclopedia}\gdef\@ISSN{2673-8392}\gdef\@continuouspages{yes}}
\DeclareOption{endocrines}{\gdef\@journal{endocrines}\gdef\@journalfull{Endocrines}\gdef\@journalshort{Endocrines}\gdef\@doiabbr{endocrines}\gdef\@ISSN{2673-396X}\gdef\@continuouspages{yes}}
\DeclareOption{energies}{\gdef\@journal{energies}\gdef\@journalfull{Energies}\gdef\@journalshort{Energies}\gdef\@doiabbr{en}\gdef\@ISSN{1996-1073}}
\DeclareOption{eng}{\gdef\@journal{eng}\gdef\@journalfull{Eng}\gdef\@journalshort{Eng}\gdef\@doiabbr{eng}\gdef\@ISSN{2673-4117}\gdef\@continuouspages{yes}}
\DeclareOption{engproc}{\gdef\@journal{engproc}\gdef\@journalfull{Engineering Proceedings}\gdef\@journalshort{Eng. Proc.}\gdef\@doiabbr{engproc}\gdef\@ISSN{2673-4591}}
%\DeclareOption{ent}{\gdef\@journal{ent}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{entomology}{\gdef\@journal{entomology}\gdef\@journalfull{Entomology}\gdef\@journalshort{Entomology}\gdef\@doiabbr{entomology}\gdef\@ISSN{2813-0502}\gdef\@continuouspages{yes}}	
\DeclareOption{entropy}{\gdef\@journal{entropy}\gdef\@journalfull{Entropy}\gdef\@journalshort{Entropy}\gdef\@doiabbr{e}\gdef\@ISSN{1099-4300}}
\DeclareOption{environments}{\gdef\@journal{environments}\gdef\@journalfull{Environments}\gdef\@journalshort{Environments}\gdef\@doiabbr{environments}\gdef\@ISSN{2076-3298}}
\DeclareOption{environsciproc}{\gdef\@journal{environsciproc}\gdef\@journalfull{Environmental Sciences Proceedings}\gdef\@journalshort{Environ. Sci. Proc.}\gdef\@doiabbr{environsciproc}\gdef\@ISSN{2673-4931}}
\DeclareOption{epidemiologia}{\gdef\@journal{epidemiologia}\gdef\@journalfull{Epidemiologia}\gdef\@journalshort{Epidemiologia}\gdef\@doiabbr{epidemiologia}\gdef\@ISSN{2673-3986}\gdef\@continuouspages{yes}}
\DeclareOption{epigenomes}{\gdef\@journal{epigenomes}\gdef\@journalfull{Epigenomes}\gdef\@journalshort{Epigenomes}\gdef\@doiabbr{epigenomes}\gdef\@ISSN{2075-4655}}
\DeclareOption{est}{\gdef\@journal{est}\gdef\@journalfull{Electrochemical Science and Technology}\gdef\@journalshort{Electrochem. Sci. Technol.}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{fermentation}{\gdef\@journal{fermentation}\gdef\@journalfull{Fermentation}\gdef\@journalshort{Fermentation}\gdef\@doiabbr{fermentation}\gdef\@ISSN{2311-5637}}
\DeclareOption{fibers}{\gdef\@journal{fibers}\gdef\@journalfull{Fibers}\gdef\@journalshort{Fibers}\gdef\@doiabbr{fib}\gdef\@ISSN{2079-6439}}
\DeclareOption{fintech}{\gdef\@journal{fintech}\gdef\@journalfull{FinTech}\gdef\@journalshort{FinTech}\gdef\@doiabbr{fintech}\gdef\@ISSN{2674-1032}\gdef\@continuouspages{yes}}
\DeclareOption{fire}{\gdef\@journal{fire}\gdef\@journalfull{Fire}\gdef\@journalshort{Fire}\gdef\@doiabbr{fire}\gdef\@ISSN{2571-6255}}
\DeclareOption{fishes}{\gdef\@journal{fishes}\gdef\@journalfull{Fishes}\gdef\@journalshort{Fishes}\gdef\@doiabbr{fishes}\gdef\@ISSN{2410-3888}}
\DeclareOption{fluids}{\gdef\@journal{fluids}\gdef\@journalfull{Fluids}\gdef\@journalshort{Fluids}\gdef\@doiabbr{fluids}\gdef\@ISSN{2311-5521}}
\DeclareOption{foods}{\gdef\@journal{foods}\gdef\@journalfull{Foods}\gdef\@journalshort{Foods}\gdef\@doiabbr{foods}\gdef\@ISSN{2304-8158}}
\DeclareOption{forecasting}{\gdef\@journal{forecasting}\gdef\@journalfull{Forecasting}\gdef\@journalshort{Forecasting}\gdef\@doiabbr{forecast}\gdef\@ISSN{2571-9394}\gdef\@continuouspages{yes}}
\DeclareOption{forensicsci}{\gdef\@journal{forensicsci}\gdef\@journalfull{Forensic Sciences}\gdef\@journalshort{Forensic Sci.}\gdef\@doiabbr{forensicsci}\gdef\@ISSN{2673-6756}\gdef\@continuouspages{yes}}
\DeclareOption{forests}{\gdef\@journal{forests}\gdef\@journalfull{Forests}\gdef\@journalshort{Forests}\gdef\@doiabbr{f}\gdef\@ISSN{1999-4907}}
\DeclareOption{fossstud}{\gdef\@journal{fossstud}\gdef\@journalfull{Fossil Studies}\gdef\@journalshort{Foss. Stud.}\gdef\@doiabbr{fossils}\gdef\@ISSN{2813-6284}\gdef\@continuouspages{yes}}
\DeclareOption{foundations}{\gdef\@journal{foundations}\gdef\@journalfull{Foundations}\gdef\@journalshort{Foundations}\gdef\@doiabbr{foundations}\gdef\@ISSN{2673-9321}\gdef\@continuouspages{yes}}
\DeclareOption{fractalfract}{\gdef\@journal{fractalfract}\gdef\@journalfull{Fractal and Fractional}\gdef\@journalshort{Fractal Fract.}\gdef\@doiabbr{fractalfract}\gdef\@ISSN{2504-3110}}
\DeclareOption{fuels}{\gdef\@journal{fuels}\gdef\@journalfull{Fuels}\gdef\@journalshort{Fuels}\gdef\@doiabbr{fuels}\gdef\@ISSN{2673-3994}\gdef\@continuouspages{yes}}
\DeclareOption{future}{\gdef\@journal{future}\gdef\@journalfull{Future}\gdef\@journalshort{Future}\gdef\@doiabbr{future}\gdef\@ISSN{2813-2882}\gdef\@continuouspages{yes}}
\DeclareOption{futureinternet}{\gdef\@journal{futureinternet}\gdef\@journalfull{Future Internet}\gdef\@journalshort{Future Internet}\gdef\@doiabbr{fi}\gdef\@ISSN{1999-5903}}
%\DeclareOption{futureparasites}{\gdef\@journal{futureparasites}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{futurepharmacol}{\gdef\@journal{futurepharmacol}\gdef\@journalfull{Future Pharmacology}\gdef\@journalshort{Future Pharmacol.}\gdef\@doiabbr{futurepharmacol}\gdef\@ISSN{2673-9879}\gdef\@continuouspages{yes}}
\DeclareOption{futurephys}{\gdef\@journal{futurephys}\gdef\@journalfull{Future Physics}\gdef\@journalshort{Future Phys.}\gdef\@doiabbr{futurephys}\gdef\@ISSN{2624-6503}}
\DeclareOption{futuretransp}{\gdef\@journal{futuretransp}\gdef\@journalfull{Future Transportation}\gdef\@journalshort{Future Transp.}\gdef\@doiabbr{futuretransp}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{galaxies}{\gdef\@journal{galaxies}\gdef\@journalfull{Galaxies}\gdef\@journalshort{Galaxies}\gdef\@doiabbr{galaxies}\gdef\@ISSN{2075-4434}}
\DeclareOption{games}{\gdef\@journal{games}\gdef\@journalfull{Games}\gdef\@journalshort{Games}\gdef\@doiabbr{g}\gdef\@ISSN{2073-4336}}
\DeclareOption{gases}{\gdef\@journal{gases}\gdef\@journalfull{Gases}\gdef\@journalshort{Gases}\gdef\@doiabbr{gases}\gdef\@ISSN{2673-5628}\gdef\@continuouspages{yes}}
\DeclareOption{gastroent}{\gdef\@journal{gastroent}\gdef\@journalfull{Gastroenterology Insights}\gdef\@journalshort{Gastroenterol. Insights}\gdef\@doiabbr{gastroent}\gdef\@ISSN{2036-7422}\gdef\@continuouspages{yes}}
\DeclareOption{gastrointestdisord}{\gdef\@journal{gastrointestdisord}\gdef\@journalfull{Gastrointestinal Disorders}\gdef\@journalshort{Gastrointest. Disord.}\gdef\@doiabbr{gidisord}\gdef\@ISSN{2624-5647}\gdef\@continuouspages{yes}}
\DeclareOption{gastronomy}{\gdef\@journal{gastronomy}\gdef\@journalfull{Gastronomy}\gdef\@journalshort{Gastronomy}\gdef\@doiabbr{gastronomy}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{gels}{\gdef\@journal{gels}\gdef\@journalfull{Gels}\gdef\@journalshort{Gels}\gdef\@doiabbr{gels}\gdef\@ISSN{2310-2861}}
\DeclareOption{genealogy}{\gdef\@journal{genealogy}\gdef\@journalfull{Genealogy}\gdef\@journalshort{Genealogy}\gdef\@doiabbr{genealogy}\gdef\@ISSN{2313-5778}}
\DeclareOption{genes}{\gdef\@journal{genes}\gdef\@journalfull{Genes}\gdef\@journalshort{Genes}\gdef\@doiabbr{genes}\gdef\@ISSN{2073-4425}}
\DeclareOption{geographies}{\gdef\@journal{geographies}\gdef\@journalfull{Geographies}\gdef\@journalshort{Geographies}\gdef\@doiabbr{geographies}\gdef\@ISSN{2673-7086}\gdef\@continuouspages{yes}}
\DeclareOption{geohazards}{\gdef\@journal{geohazards}\gdef\@journalfull{GeoHazards}\gdef\@journalshort{GeoHazards}\gdef\@doiabbr{geohazards}\gdef\@ISSN{2624-795X}\gdef\@continuouspages{yes}}
\DeclareOption{geomatics}{\gdef\@journal{geomatics}\gdef\@journalfull{Geomatics}\gdef\@journalshort{Geomatics}\gdef\@doiabbr{geomatics}\gdef\@ISSN{2673-7418}\gdef\@continuouspages{yes}}
\DeclareOption{geometry}{\gdef\@journal{geometry}\gdef\@journalfull{Geometry}\gdef\@journalshort{Geometry}\gdef\@doiabbr{geometry}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{geosciences}{\gdef\@journal{geosciences}\gdef\@journalfull{Geosciences}\gdef\@journalshort{Geosciences}\gdef\@doiabbr{geosciences}\gdef\@ISSN{2076-3263}}
\DeclareOption{geotechnics}{\gdef\@journal{geotechnics}\gdef\@journalfull{Geotechnics}\gdef\@journalshort{Geotechnics}\gdef\@doiabbr{geotechnics}\gdef\@ISSN{2673-7094}\gdef\@continuouspages{yes}}
\DeclareOption{geriatrics}{\gdef\@journal{geriatrics}\gdef\@journalfull{Geriatrics}\gdef\@journalshort{Geriatrics}\gdef\@doiabbr{geriatrics}\gdef\@ISSN{2308-3417}}
\DeclareOption{grasses}{\gdef\@journal{grasses}\gdef\@journalfull{Grasses}\gdef\@journalshort{Grasses}\gdef\@doiabbr{grasses}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{gucdd}{\gdef\@journal{gucdd}\gdef\@journalfull{Gout, Urate, and Crystal Deposition Disease}\gdef\@journalshort{Gout Urate Cryst. Depos. Dis.}\gdef\@doiabbr{gucdd}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hardware}{\gdef\@journal{hardware}\gdef\@journalfull{Hardware}\gdef\@journalshort{Hardware}\gdef\@doiabbr{hardware}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hazardousmatters}{\gdef\@journal{hazardousmatters}\gdef\@journalfull{Hazardous Matters}\gdef\@journalshort{Hazard. Matters}\gdef\@doiabbr{}\gdef\@ISSN{0014-0014}}
\DeclareOption{healthcare}{\gdef\@journal{healthcare}\gdef\@journalfull{Healthcare}\gdef\@journalshort{Healthcare}\gdef\@doiabbr{healthcare}\gdef\@ISSN{2227-9032}}
\DeclareOption{hearts}{\gdef\@journal{hearts}\gdef\@journalfull{Hearts}\gdef\@journalshort{Hearts}\gdef\@doiabbr{hearts}\gdef\@ISSN{2673-3846}\gdef\@continuouspages{yes}}
\DeclareOption{hemato}{\gdef\@journal{hemato}\gdef\@journalfull{Hemato}\gdef\@journalshort{Hemato}\gdef\@doiabbr{hemato}\gdef\@ISSN{2673-6357}\gdef\@continuouspages{yes}}
\DeclareOption{hematolrep}{\gdef\@journal{hematolrep}\gdef\@journalfull{Hematology Reports}\gdef\@journalshort{Hematol. Rep.}\gdef\@doiabbr{hematolrep}\gdef\@ISSN{2038-8330}\gdef\@continuouspages{yes}}
\DeclareOption{heritage}{\gdef\@journal{heritage}\gdef\@journalfull{Heritage}\gdef\@journalshort{Heritage}\gdef\@doiabbr{heritage}\gdef\@ISSN{2571-9408}\gdef\@continuouspages{yes}}
\DeclareOption{higheredu}{\gdef\@journal{higheredu}\gdef\@journalfull{Trends in Higher Education}\gdef\@journalshort{Trends High. Educ.}\gdef\@doiabbr{higheredu}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{highthroughput}{\gdef\@journal{highthroughput}\gdef\@journalfull{High-Throughput}\gdef\@journalshort{High-Throughput}\gdef\@doiabbr{ht}\gdef\@ISSN{2571-5135}}
\DeclareOption{histories}{\gdef\@journal{histories}\gdef\@journalfull{Histories}\gdef\@journalshort{Histories}\gdef\@doiabbr{histories}\gdef\@ISSN{2409-9252}\gdef\@continuouspages{yes}}
\DeclareOption{horticulturae}{\gdef\@journal{horticulturae}\gdef\@journalfull{Horticulturae}\gdef\@journalshort{Horticulturae}\gdef\@doiabbr{horticulturae}\gdef\@ISSN{2311-7524}}
\DeclareOption{hospitals}{\gdef\@journal{hospitals}\gdef\@journalfull{Hospitals}\gdef\@journalshort{Hospitals}\gdef\@doiabbr{hospitals}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{humanities}{\gdef\@journal{humanities}\gdef\@journalfull{Humanities}\gdef\@journalshort{Humanities}\gdef\@doiabbr{h}\gdef\@ISSN{2076-0787}}
\DeclareOption{humans}{\gdef\@journal{humans}\gdef\@journalfull{Humans}\gdef\@journalshort{Humans}\gdef\@doiabbr{humans}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{hydrobiology}{\gdef\@journal{hydrobiology}\gdef\@journalfull{Hydrobiology}\gdef\@journalshort{Hydrobiology	}\gdef\@doiabbr{hydrobiology}\gdef\@ISSN{2673-9917}\gdef\@continuouspages{yes}}
\DeclareOption{hydrogen}{\gdef\@journal{hydrogen}\gdef\@journalfull{Hydrogen}\gdef\@journalshort{Hydrogen}\gdef\@doiabbr{hydrogen}\gdef\@ISSN{2673-4141}\gdef\@continuouspages{yes}}
\DeclareOption{hydrology}{\gdef\@journal{hydrology}\gdef\@journalfull{Hydrology}\gdef\@journalshort{Hydrology}\gdef\@doiabbr{hydrology}\gdef\@ISSN{2306-5338}}
\DeclareOption{hygiene}{\gdef\@journal{hygiene}\gdef\@journalfull{Hygiene}\gdef\@journalshort{Hygiene}\gdef\@doiabbr{hygiene}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{glacies}{\gdef\@journal{glacies}\gdef\@journalfull{Glacies}\gdef\@journalshort{Glacies}\gdef\@doiabbr{glacies}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{idr}{\gdef\@journal{idr}\gdef\@journalfull{Infectious Disease Reports}\gdef\@journalshort{Infect. Dis. Rep.}\gdef\@doiabbr{idr}\gdef\@ISSN{2036-7449}\gdef\@continuouspages{yes}}
\DeclareOption{ijerph}{\gdef\@journal{ijerph}\gdef\@journalfull{International Journal of Environmental Research and Public Health}\gdef\@journalshort{Int. J. Environ. Res. Public Health}\gdef\@doiabbr{ijerph}\gdef\@ISSN{1660-4601}}
\DeclareOption{ijfs}{\gdef\@journal{ijfs}\gdef\@journalfull{International Journal of Financial Studies}\gdef\@journalshort{Int. J. Financial Stud.}\gdef\@doiabbr{ijfs}\gdef\@ISSN{2227-7072}}
\DeclareOption{ijgi}{\gdef\@journal{ijgi}\gdef\@journalfull{ISPRS International Journal of Geo-Information}\gdef\@journalshort{ISPRS Int. J. Geo-Inf.}\gdef\@doiabbr{ijgi}\gdef\@ISSN{2220-9964}}
\DeclareOption{ijmd}{\gdef\@journal{ijmd}\gdef\@journalfull{International Journal of Medical Devices}\gdef\@journalshort{Int. J. Med. Devices}\gdef\@doiabbr{ijmd}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{ijms}{\gdef\@journal{ijms}\gdef\@journalfull{International Journal of Molecular Sciences}\gdef\@journalshort{Int. J. Mol. Sci.}\gdef\@doiabbr{ijms}\gdef\@ISSN{1422-0067}}
\DeclareOption{ijns}{\gdef\@journal{ijns}\gdef\@journalfull{International Journal of Neonatal Screening}\gdef\@journalshort{Int. J. Neonatal Screen.}\gdef\@doiabbr{ijns}\gdef\@ISSN{2409-515X}}
\DeclareOption{ijpb}{\gdef\@journal{ijpb}\gdef\@journalfull{International Journal of Plant Biology}\gdef\@journalshort{Int. J. Plant Biol.}\gdef\@doiabbr{ijpb}\gdef\@ISSN{2037-0164}\gdef\@continuouspages{yes}}
\DeclareOption{ijt}{\gdef\@journal{ijt}\gdef\@journalfull{International Journal of Topology}\gdef\@journalshort{Int. J. Topol.}\gdef\@doiabbr{ijt}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{ijtm}{\gdef\@journal{ijtm}\gdef\@journalfull{International Journal of Translational Medicine}\gdef\@journalshort{Int. J. Transl. Med.}\gdef\@doiabbr{ijtm}\gdef\@ISSN{2673-8937}\gdef\@continuouspages{yes}}
\DeclareOption{ijtpp}{\gdef\@journal{ijtpp}\gdef\@journalfull{International Journal of Turbomachinery, Propulsion and Power}\gdef\@journalshort{Int. J. Turbomach. Propuls. Power}\gdef\@doiabbr{ijtpp}\gdef\@ISSN{2504-186X}}
\DeclareOption{ime}{\gdef\@journal{ime}\gdef\@journalfull{International Medical Education}\gdef\@journalshort{Int. Med. Educ.}\gdef\@doiabbr{ime}\gdef\@ISSN{2813-141X}\gdef\@continuouspages{yes}}
\DeclareOption{immuno}{\gdef\@journal{immuno}\gdef\@journalfull{Immuno}\gdef\@journalshort{Immuno}\gdef\@doiabbr{immuno}\gdef\@ISSN{2673-5601}\gdef\@continuouspages{yes}}
\DeclareOption{informatics}{\gdef\@journal{informatics}\gdef\@journalfull{Informatics}\gdef\@journalshort{Informatics}\gdef\@doiabbr{informatics}\gdef\@ISSN{2227-9709}}
\DeclareOption{information}{\gdef\@journal{information}\gdef\@journalfull{Information}\gdef\@journalshort{Information}\gdef\@doiabbr{info}\gdef\@ISSN{2078-2489}}
\DeclareOption{infrastructures}{\gdef\@journal{infrastructures}\gdef\@journalfull{Infrastructures}\gdef\@journalshort{Infrastructures}\gdef\@doiabbr{infrastructures}\gdef\@ISSN{2412-3811}}
\DeclareOption{inorganics}{\gdef\@journal{inorganics}\gdef\@journalfull{Inorganics}\gdef\@journalshort{Inorganics}\gdef\@doiabbr{inorganics}\gdef\@ISSN{2304-6740}}
\DeclareOption{insects}{\gdef\@journal{insects}\gdef\@journalfull{Insects}\gdef\@journalshort{Insects}\gdef\@doiabbr{insects}\gdef\@ISSN{2075-4450}}
\DeclareOption{instruments}{\gdef\@journal{instruments}\gdef\@journalfull{Instruments}\gdef\@journalshort{Instruments}\gdef\@doiabbr{instruments}\gdef\@ISSN{2410-390X}}
\DeclareOption{inventions}{\gdef\@journal{inventions}\gdef\@journalfull{Inventions}\gdef\@journalshort{Inventions}\gdef\@doiabbr{inventions}\gdef\@ISSN{2411-5134}}
\DeclareOption{iot}{\gdef\@journal{iot}\gdef\@journalfull{IoT}\gdef\@journalshort{IoT}\gdef\@doiabbr{iot}\gdef\@ISSN{2624-831X}\gdef\@continuouspages{yes}}
\DeclareOption{j}{\gdef\@journal{j}\gdef\@journalfull{J}\gdef\@journalshort{J}\gdef\@doiabbr{j}\gdef\@ISSN{2571-8800}\gdef\@continuouspages{yes}}
\DeclareOption{jal}{\gdef\@journal{jal}\gdef\@journalfull{Journal of Ageing and Longevity}\gdef\@journalshort{J. Ageing Longev.}\gdef\@doiabbr{jal}\gdef\@ISSN{2673-9259}\gdef\@continuouspages{yes}}
\DeclareOption{jcdd}{\gdef\@journal{jcdd}\gdef\@journalfull{Journal of Cardiovascular Development and Disease}\gdef\@journalshort{J. Cardiovasc. Dev. Dis.}\gdef\@doiabbr{jcdd}\gdef\@ISSN{2308-3425}}
\DeclareOption{jcm}{\gdef\@journal{jcm}\gdef\@journalfull{Journal of Clinical Medicine}\gdef\@journalshort{J. Clin. Med.}\gdef\@doiabbr{jcm}\gdef\@ISSN{2077-0383}}
\DeclareOption{jcp}{\gdef\@journal{jcp}\gdef\@journalfull{Journal of Cybersecurity and Privacy}\gdef\@journalshort{J. Cybersecur. Priv.}\gdef\@doiabbr{jcp}\gdef\@ISSN{2624-800X}\gdef\@continuouspages{yes}}
\DeclareOption{jcs}{\gdef\@journal{jcs}\gdef\@journalfull{Journal of Composites Science}\gdef\@journalshort{J. Compos. Sci.}\gdef\@doiabbr{jcs}\gdef\@ISSN{2504-477X}}
\DeclareOption{jcto}{\gdef\@journal{jcto}\gdef\@journalfull{Journal of Clinical \& Translational Ophthalmology}\gdef\@journalshort{J. Clin. Transl. Ophthalmol.}\gdef\@doiabbr{jcto}\gdef\@ISSN{2813-1053}\gdef\@continuouspages{yes}}
\DeclareOption{jdad}{\gdef\@journal{jdad}\gdef\@journalfull{Journal of Dementia and Alzheimer's Disease}\gdef\@journalshort{J. Dement. Alzheimer's Dis.}\gdef\@doiabbr{jdad}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jdb}{\gdef\@journal{jdb}\gdef\@journalfull{Journal of Developmental Biology}\gdef\@journalshort{J. Dev. Biol.}\gdef\@doiabbr{jdb}\gdef\@ISSN{2221-3759}}
\DeclareOption{jeta}{\gdef\@journal{jeta}\gdef\@journalfull{Journal of Experimental and Theoretical Analyses}\gdef\@journalshort{J. Exp. Theor. Anal.}\gdef\@doiabbr{jeta}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jfb}{\gdef\@journal{jfb}\gdef\@journalfull{Journal of Functional Biomaterials}\gdef\@journalshort{J. Funct. Biomater.}\gdef\@doiabbr{jfb}\gdef\@ISSN{2079-4983}}
\DeclareOption{jfmk}{\gdef\@journal{jfmk}\gdef\@journalfull{Journal of Functional Morphology and Kinesiology}\gdef\@journalshort{J. Funct. Morphol. Kinesiol.}\gdef\@doiabbr{jfmk}\gdef\@ISSN{2411-5142}}
\DeclareOption{jimaging}{\gdef\@journal{jimaging}\gdef\@journalfull{Journal of Imaging}\gdef\@journalshort{J. Imaging}\gdef\@doiabbr{jimaging}\gdef\@ISSN{2313-433X}}
\DeclareOption{jintelligence}{\gdef\@journal{jintelligence}\gdef\@journalfull{Journal of Intelligence}\gdef\@journalshort{J. Intell.}\gdef\@doiabbr{jintelligence}\gdef\@ISSN{2079-3200}}
\DeclareOption{jlpea}{\gdef\@journal{jlpea}\gdef\@journalfull{Journal of Low Power Electronics and Applications}\gdef\@journalshort{J. Low Power Electron. Appl.}\gdef\@doiabbr{jlpea}\gdef\@ISSN{2079-9268}}
\DeclareOption{jmahp}{\gdef\@journal{jmahp}\gdef\@journalfull{Journal of Market Access \& Health Policy}\gdef\@journalshort{	. Mark. Access Health Policy}\gdef\@doiabbr{jmahp}\gdef\@ISSN{2001-6689}\gdef\@continuouspages{yes}}
\DeclareOption{jmmp}{\gdef\@journal{jmmp}\gdef\@journalfull{Journal of Manufacturing and Materials Processing}\gdef\@journalshort{J. Manuf. Mater. Process.}\gdef\@doiabbr{jmmp}\gdef\@ISSN{2504-4494}}
\DeclareOption{jmp}{\gdef\@journal{jmp}\gdef\@journalfull{Journal of Molecular Pathology}\gdef\@journalshort{J. Mol. Pathol.}\gdef\@doiabbr{jmp}\gdef\@ISSN{2673-5261}\gdef\@continuouspages{yes}}
\DeclareOption{jmse}{\gdef\@journal{jmse}\gdef\@journalfull{Journal of Marine Science and Engineering}\gdef\@journalshort{J. Mar. Sci. Eng.}\gdef\@doiabbr{jmse}\gdef\@ISSN{2077-1312}}
\DeclareOption{jne}{\gdef\@journal{jne}\gdef\@journalfull{Journal of Nuclear Engineering}\gdef\@journalshort{J. Nucl. Eng.}\gdef\@doiabbr{jne}\gdef\@ISSN{2673-4362}\gdef\@continuouspages{yes}}
\DeclareOption{jnt}{\gdef\@journal{jnt}\gdef\@journalfull{Journal of Nanotheranostics}\gdef\@journalshort{J. Nanotheranostics}\gdef\@doiabbr{jnt}\gdef\@ISSN{2624-845X}\gdef\@continuouspages{yes}}
\DeclareOption{jof}{\gdef\@journal{jof}\gdef\@journalfull{Journal of Fungi}\gdef\@journalshort{J. Fungi}\gdef\@doiabbr{jof}\gdef\@ISSN{2309-608X}}
\DeclareOption{joitmc}{\gdef\@journal{joitmc}\gdef\@journalfull{Journal of Open Innovation: Technology, Market, and Complexity}\gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}\gdef\@doiabbr{joitmc}\gdef\@ISSN{2199-8531}}
\DeclareOption{joma}{\gdef\@journal{joma}\gdef\@journalfull{Journal of the Oman Medical Association}\gdef\@journalshort{J. Oman Med. Assoc.}\gdef\@doiabbr{joma}\gdef\@ISSN{2813-8759}\gdef\@continuouspages{yes}}
\DeclareOption{jor}{\gdef\@journal{jor}\gdef\@journalfull{Journal of Respiration}\gdef\@journalshort{J. Respir.}\gdef\@doiabbr{jor}\gdef\@ISSN{2673-527X}\gdef\@continuouspages{yes}}
\DeclareOption{journalmedia}{\gdef\@journal{journalmedia}\gdef\@journalfull{Journalism and Media}\gdef\@journalshort{Journal. Media}\gdef\@doiabbr{journalmedia}\gdef\@ISSN{2673-5172}\gdef\@continuouspages{yes}}
\DeclareOption{jox}{\gdef\@journal{jox}\gdef\@journalfull{Journal of Xenobiotics}\gdef\@journalshort{J. Xenobiot.}\gdef\@doiabbr{jox}\gdef\@ISSN{2039-4713}\gdef\@continuouspages{yes}}
\DeclareOption{jpbi}{\gdef\@journal{jpbi}\gdef\@journalfull{Journal of Pharmaceutical and BioTech Industry}\gdef\@journalshort{J. Pharm. BioTech Ind.}\gdef\@doiabbr{jpbi}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jpm}{\gdef\@journal{jpm}\gdef\@journalfull{Journal of Personalized Medicine}\gdef\@journalshort{J. Pers. Med.}\gdef\@doiabbr{jpm}\gdef\@ISSN{2075-4426}}
\DeclareOption{jrfm}{\gdef\@journal{jrfm}\gdef\@journalfull{Journal of Risk and Financial Management}\gdef\@journalshort{J. Risk Financial Manag.}\gdef\@doiabbr{jrfm}\gdef\@ISSN{1911-8074}}
\DeclareOption{jsan}{\gdef\@journal{jsan}\gdef\@journalfull{Journal of Sensor and Actuator Networks}\gdef\@journalshort{J. Sens. Actuator Netw.}\gdef\@doiabbr{jsan}\gdef\@ISSN{2224-2708}}
\DeclareOption{jtaer}{\gdef\@journal{jtaer}\gdef\@journalfull{Journal of Theoretical and Applied Electronic Commerce Research}\gdef\@journalshort{J. Theor. Appl. Electron. Commer. Res.}\gdef\@doiabbr{jtaer}\gdef\@ISSN{0718-1876}\gdef\@continuouspages{yes}}
\DeclareOption{jvd}{\gdef\@journal{jvd}\gdef\@journalfull{Journal of Vascular Diseases}\gdef\@journalshort{JVD}\gdef\@doiabbr{jvd}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{jzbg}{\gdef\@journal{jzbg}\gdef\@journalfull{Journal of Zoological and Botanical Gardens}\gdef\@journalshort{J. Zool. Bot. Gard.}\gdef\@doiabbr{jzbg}\gdef\@ISSN{2673-5636}\gdef\@continuouspages{yes}}
%\DeclareOption{kidney}{\gdef\@journal{kidney}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{kidneydial}{\gdef\@journal{kidneydial}\gdef\@journalfull{Kidney and Dialysis}\gdef\@journalshort{Kidney Dial.}\gdef\@doiabbr{kinasesphosphatases}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{kinasesphosphatases}{\gdef\@journal{kinasesphosphatases}\gdef\@journalfull{Kinases and Phosphatases}\gdef\@journalshort{Kinases Phosphatases}\gdef\@doiabbr{kinasesphosphatases}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{knowledge}{\gdef\@journal{knowledge}\gdef\@journalfull{Knowledge}\gdef\@journalshort{Knowledge}\gdef\@doiabbr{knowledge}\gdef\@ISSN{2673-9585}\gdef\@continuouspages{yes}}
\DeclareOption{laboratories}{\gdef\@journal{laboratories}\gdef\@journalfull{Laboratories}\gdef\@journalshort{Laboratories}\gdef\@doiabbr{laboratories}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{land}{\gdef\@journal{land}\gdef\@journalfull{Land}\gdef\@journalshort{Land}\gdef\@doiabbr{land}\gdef\@ISSN{2073-445X}}
\DeclareOption{languages}{\gdef\@journal{languages}\gdef\@journalfull{Languages}\gdef\@journalshort{Languages}\gdef\@doiabbr{languages}\gdef\@ISSN{2226-471X}}
\DeclareOption{laws}{\gdef\@journal{laws}\gdef\@journalfull{Laws}\gdef\@journalshort{Laws}\gdef\@doiabbr{laws}\gdef\@ISSN{2075-471X}}
\DeclareOption{life}{\gdef\@journal{life}\gdef\@journalfull{Life}\gdef\@journalshort{Life}\gdef\@doiabbr{life}\gdef\@ISSN{2075-1729}}
\DeclareOption{limnolrev}{\gdef\@journal{limnolrev}\gdef\@journalfull{Limnological Review}\gdef\@journalshort{Limnol. Rev.}\gdef\@doiabbr{limnolrev}\gdef\@ISSN{2300-7575}\gdef\@continuouspages{yes}}
\DeclareOption{lipidology}{\gdef\@journal{lipidology}\gdef\@journalfull{Lipidology}\gdef\@journalshort{Lipidology}\gdef\@doiabbr{lipidology}\gdef\@ISSN{2813-7086}\gdef\@continuouspages{yes}}
\DeclareOption{liquids}{\gdef\@journal{liquids}\gdef\@journalfull{Liquids}\gdef\@journalshort{Liquids}\gdef\@doiabbr{liquids}\gdef\@ISSN{2673-8015}\gdef\@continuouspages{yes}}
\DeclareOption{literature}{\gdef\@journal{literature}\gdef\@journalfull{Literature}\gdef\@journalshort{Literature}\gdef\@doiabbr{literature}\gdef\@ISSN{2410-9789}\gdef\@continuouspages{yes}}
\DeclareOption{livers}{\gdef\@journal{livers}\gdef\@journalfull{Livers}\gdef\@journalshort{Livers}\gdef\@doiabbr{livers}\gdef\@ISSN{2673-4389}\gdef\@continuouspages{yes}}
\DeclareOption{logics}{\gdef\@journal{logics}\gdef\@journalfull{Logics}\gdef\@journalshort{Logics}\gdef\@doiabbr{logics}\gdef\@ISSN{2813-0405}\gdef\@continuouspages{yes}}
\DeclareOption{logistics}{\gdef\@journal{logistics}\gdef\@journalfull{Logistics}\gdef\@journalshort{Logistics}\gdef\@doiabbr{logistics}\gdef\@ISSN{2305-6290}}
\DeclareOption{lubricants}{\gdef\@journal{lubricants}\gdef\@journalfull{Lubricants}\gdef\@journalshort{Lubricants}\gdef\@doiabbr{lubricants}\gdef\@ISSN{2075-4442}}
\DeclareOption{lymphatics}{\gdef\@journal{lymphatics}\gdef\@journalfull{Lymphatics}\gdef\@journalshort{Lymphatics}\gdef\@doiabbr{lymphatics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}	
\DeclareOption{machines}{\gdef\@journal{machines}\gdef\@journalfull{Machines}\gdef\@journalshort{Machines}\gdef\@doiabbr{machines}\gdef\@ISSN{2075-1702}}
\DeclareOption{macromol}{\gdef\@journal{macromol}\gdef\@journalfull{Macromol}\gdef\@journalshort{Macromol}\gdef\@doiabbr{macromol}\gdef\@ISSN{2673-6209}\gdef\@continuouspages{yes}}
\DeclareOption{magnetism}{\gdef\@journal{magnetism}\gdef\@journalfull{Magnetism}\gdef\@journalshort{Magnetism}\gdef\@doiabbr{magnetism}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{magnetochemistry}{\gdef\@journal{magnetochemistry}\gdef\@journalfull{Magnetochemistry}\gdef\@journalshort{Magnetochemistry}\gdef\@doiabbr{magnetochemistry}\gdef\@ISSN{2312-7481}}
\DeclareOption{make}{\gdef\@journal{make}\gdef\@journalfull{Machine Learning and Knowledge Extraction}\gdef\@journalshort{Mach. Learn. Knowl. Extr.}\gdef\@doiabbr{make}\gdef\@ISSN{2504-4990}\gdef\@continuouspages{yes}}
\DeclareOption{marinedrugs}{\gdef\@journal{marinedrugs}\gdef\@journalfull{Marine Drugs}\gdef\@journalshort{Mar. Drugs}\gdef\@doiabbr{md}\gdef\@ISSN{1660-3397}}
\DeclareOption{materials}{\gdef\@journal{materials}\gdef\@journalfull{Materials}\gdef\@journalshort{Materials}\gdef\@doiabbr{ma}\gdef\@ISSN{1996-1944}}
\DeclareOption{materproc}{\gdef\@journal{materproc}\gdef\@journalfull{Materials Proceedings}\gdef\@journalshort{Mater. Proc.}\gdef\@doiabbr{materproc}\gdef\@ISSN{2673-4605}}
\DeclareOption{mathematics}{\gdef\@journal{mathematics}\gdef\@journalfull{Mathematics}\gdef\@journalshort{Mathematics}\gdef\@doiabbr{math}\gdef\@ISSN{2227-7390}}
\DeclareOption{mca}{\gdef\@journal{mca}\gdef\@journalfull{Mathematical and Computational Applications}\gdef\@journalshort{Math. Comput. Appl.}\gdef\@doiabbr{mca}\gdef\@ISSN{2297-8747}}
\DeclareOption{measurements}{\gdef\@journal{measurements}\gdef\@journalfull{Measurements}\gdef\@journalshort{Measurements}\gdef\@doiabbr{measurements}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{medicina}{\gdef\@journal{medicina}\gdef\@journalfull{Medicina}\gdef\@journalshort{Medicina}\gdef\@doiabbr{medicina}\gdef\@ISSN{1648-9144}}
\DeclareOption{medicines}{\gdef\@journal{medicines}\gdef\@journalfull{Medicines}\gdef\@journalshort{Medicines}\gdef\@doiabbr{medicines}\gdef\@ISSN{2305-6320}}
\DeclareOption{medsci}{\gdef\@journal{medsci}\gdef\@journalfull{Medical Sciences}\gdef\@journalshort{Med. Sci.}\gdef\@doiabbr{medsci}\gdef\@ISSN{2076-3271}}
\DeclareOption{membranes}{\gdef\@journal{membranes}\gdef\@journalfull{Membranes}\gdef\@journalshort{Membranes}\gdef\@doiabbr{membranes}\gdef\@ISSN{2077-0375}}
\DeclareOption{merits}{\gdef\@journal{merits}\gdef\@journalfull{Merits}\gdef\@journalshort{Merits}\gdef\@doiabbr{merits}\gdef\@ISSN{2673-8104}\gdef\@continuouspages{yes}}
\DeclareOption{metabolites}{\gdef\@journal{metabolites}\gdef\@journalfull{Metabolites}\gdef\@journalshort{Metabolites}\gdef\@doiabbr{metabo}\gdef\@ISSN{2218-1989}}
\DeclareOption{metals}{\gdef\@journal{metals}\gdef\@journalfull{Metals}\gdef\@journalshort{Metals}\gdef\@doiabbr{met}\gdef\@ISSN{2075-4701}}
\DeclareOption{meteorology}{\gdef\@journal{meteorology}\gdef\@journalfull{Meteorology}\gdef\@journalshort{Meteorology}\gdef\@doiabbr{meteorology}\gdef\@ISSN{2674-0494}\gdef\@continuouspages{yes}}
\DeclareOption{methane}{\gdef\@journal{methane}\gdef\@journalfull{Methane}\gdef\@journalshort{Methane}\gdef\@doiabbr{methane}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{metrology}{\gdef\@journal{metrology}\gdef\@journalfull{Metrology}\gdef\@journalshort{Metrology}\gdef\@doiabbr{metrology}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{micro}{\gdef\@journal{micro}\gdef\@journalfull{Micro}\gdef\@journalshort{Micro}\gdef\@doiabbr{micro}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{microarrays}{\gdef\@journal{microarrays}\gdef\@journalfull{Microarrays}\gdef\@journalshort{Microarrays}\gdef\@doiabbr{microarrays}\gdef\@ISSN{2076-3905}}
\DeclareOption{microbiolres}{\gdef\@journal{microbiolres}\gdef\@journalfull{Microbiology Research}\gdef\@journalshort{Microbiol. Res.}\gdef\@doiabbr{microbiolres}\gdef\@ISSN{2036-7481}\gdef\@continuouspages{yes}}
\DeclareOption{micromachines}{\gdef\@journal{micromachines}\gdef\@journalfull{Micromachines}\gdef\@journalshort{Micromachines}\gdef\@doiabbr{mi}\gdef\@ISSN{2072-666X}}
\DeclareOption{microorganisms}{\gdef\@journal{microorganisms}\gdef\@journalfull{Microorganisms}\gdef\@journalshort{Microorganisms}\gdef\@doiabbr{microorganisms}\gdef\@ISSN{2076-2607}}
\DeclareOption{microplastics}{\gdef\@journal{microplastics}\gdef\@journalfull{Microplastics}\gdef\@journalshort{Microplastics}\gdef\@doiabbr{microplastics}\gdef\@ISSN{2673-8929}\gdef\@continuouspages{yes}}
\DeclareOption{minerals}{\gdef\@journal{minerals}\gdef\@journalfull{Minerals}\gdef\@journalshort{Minerals}\gdef\@doiabbr{min}\gdef\@ISSN{2075-163X}}
\DeclareOption{mining}{\gdef\@journal{mining}\gdef\@journalfull{Mining}\gdef\@journalshort{Mining}\gdef\@doiabbr{mining}\gdef\@ISSN{2673-6489}\gdef\@continuouspages{yes}}
\DeclareOption{modelling}{\gdef\@journal{modelling}\gdef\@journalfull{Modelling}\gdef\@journalshort{Modelling}\gdef\@doiabbr{modelling}\gdef\@ISSN{2673-3951}\gdef\@continuouspages{yes}}
\DeclareOption{molbank}{\gdef\@journal{molbank}\gdef\@journalfull{Molbank}\gdef\@journalshort{Molbank}\gdef\@doiabbr{M}\gdef\@ISSN{1422-8599}}
\DeclareOption{molecules}{\gdef\@journal{molecules}\gdef\@journalfull{Molecules}\gdef\@journalshort{Molecules}\gdef\@doiabbr{molecules}\gdef\@ISSN{1420-3049}}
\DeclareOption{mps}{\gdef\@journal{mps}\gdef\@journalfull{Methods and Protocols}\gdef\@journalshort{Methods Protoc.}\gdef\@doiabbr{mps}\gdef\@ISSN{2409-9279}}
\DeclareOption{msf}{\gdef\@journal{msf}\gdef\@journalfull{Medical Sciences Forum}\gdef\@journalshort{Med. Sci. Forum}\gdef\@doiabbr{msf}\gdef\@ISSN{2673-9992}}
\DeclareOption{mti}{\gdef\@journal{mti}\gdef\@journalfull{Multimodal Technologies and Interaction}\gdef\@journalshort{Multimodal Technol. Interact.}\gdef\@doiabbr{mti}\gdef\@ISSN{2414-4088}}
\DeclareOption{muscles}{\gdef\@journal{muscles}\gdef\@journalfull{Muscles}\gdef\@journalshort{Muscles}\gdef\@doiabbr{muscles}\gdef\@ISSN{2813-0413}\gdef\@continuouspages{yes}}
\DeclareOption{nanoenergyadv}{\gdef\@journal{nanoenergyadv}\gdef\@journalfull{Nanoenergy Advances}\gdef\@journalshort{Nanoenergy Adv.}\gdef\@doiabbr{nanoenergyadv}\gdef\@ISSN{2673-706X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomanufacturing}{\gdef\@journal{nanomanufacturing}\gdef\@journalfull{Nanomanufacturing}\gdef\@journalshort{Nanomanufacturing}\gdef\@doiabbr{nanomanufacturing}\gdef\@ISSN{2673-687X}\gdef\@continuouspages{yes}}
\DeclareOption{nanomaterials}{\gdef\@journal{nanomaterials}\gdef\@journalfull{Nanomaterials}\gdef\@journalshort{Nanomaterials}\gdef\@doiabbr{nano}\gdef\@ISSN{2079-4991}}
\DeclareOption{ncrna}{\gdef\@journal{ncrna}\gdef\@journalfull{Non-Coding RNA}\gdef\@journalshort{Non-Coding RNA}\gdef\@doiabbr{ncrna}\gdef\@ISSN{2311-553X}}
\DeclareOption{ndt}{\gdef\@journal{ndt}\gdef\@journalfull{NDT}\gdef\@journalshort{NDT}\gdef\@doiabbr{ndt}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{network}{\gdef\@journal{network}\gdef\@journalfull{Network}\gdef\@journalshort{Network}\gdef\@doiabbr{network}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{neuroglia}{\gdef\@journal{neuroglia}\gdef\@journalfull{Neuroglia}\gdef\@journalshort{Neuroglia}\gdef\@doiabbr{neuroglia}\gdef\@ISSN{2571-6980}\gdef\@continuouspages{yes}}
\DeclareOption{neurolint}{\gdef\@journal{neurolint}\gdef\@journalfull{Neurology International}\gdef\@journalshort{Neurol. Int.}\gdef\@doiabbr{neurolint}\gdef\@ISSN{2035-8377}\gdef\@continuouspages{yes}}
\DeclareOption{neurosci}{\gdef\@journal{neurosci}\gdef\@journalfull{NeuroSci}\gdef\@journalshort{NeuroSci}\gdef\@doiabbr{neurosci}\gdef\@ISSN{2673-4087}\gdef\@continuouspages{yes}}
\DeclareOption{nitrogen}{\gdef\@journal{nitrogen}\gdef\@journalfull{Nitrogen}\gdef\@journalshort{Nitrogen}\gdef\@doiabbr{nitrogen}\gdef\@ISSN{2504-3129}\gdef\@continuouspages{yes}}
\DeclareOption{notspecified}{\gdef\@journal{notspecified}\gdef\@journalfull{Journal Not Specified}\gdef\@journalshort{Journal Not Specified}\gdef\@doiabbr{}\gdef\@ISSN{}}
%%\DeclareOption{nri}{\gdef\@journal{nri}\gdef\@journalfull{Natural Resources Informatics}\gdef\@journalshort{Nat. Resour. Inform.}\gdef\@doiabbr{nri}\gdef\@ISSN{2673-981X}\gdef\@continuouspages{yes}}
\DeclareOption{nursrep}{\gdef\@journal{nursrep}\gdef\@journalfull{Nursing Reports}\gdef\@journalshort{Nurs. Rep.}\gdef\@doiabbr{nursrep}\gdef\@ISSN{2039-4403}\gdef\@continuouspages{yes}}
\DeclareOption{nutraceuticals}{\gdef\@journal{nutraceuticals}\gdef\@journalfull{Nutraceuticals}\gdef\@journalshort{Nutraceuticals}\gdef\@doiabbr{nutraceuticals}\gdef\@ISSN{1661-3821}\gdef\@continuouspages{yes}}
\DeclareOption{nutrients}{\gdef\@journal{nutrients}\gdef\@journalfull{Nutrients}\gdef\@journalshort{Nutrients}\gdef\@doiabbr{nu}\gdef\@ISSN{2072-6643}}
\DeclareOption{obesities}{\gdef\@journal{obesities}\gdef\@journalfull{Obesities}\gdef\@journalshort{Obesities}\gdef\@doiabbr{obesities}\gdef\@ISSN{2673-4168}\gdef\@continuouspages{yes}}
\DeclareOption{oceans}{\gdef\@journal{oceans}\gdef\@journalfull{Oceans}\gdef\@journalshort{Oceans}\gdef\@doiabbr{oceans}\gdef\@ISSN{2673-1924}\gdef\@continuouspages{yes}}
\DeclareOption{ohbm}{\gdef\@journal{ohbm}\gdef\@journalfull{Journal of Otorhinolaryngology, Hearing and Balance Medicine}\gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}\gdef\@doiabbr{ohbm}\gdef\@ISSN{2504-463X}}
\DeclareOption{onco}{\gdef\@journal{onco}\gdef\@journalfull{Onco}\gdef\@journalshort{Onco}\gdef\@doiabbr{onco}\gdef\@ISSN{2673-7523}\gdef\@continuouspages{yes}}
%\DeclareOption{oncopathology}{\gdef\@journal{oncopathology}\gdef\@journalfull{}\gdef\@journalshort{}\gdef\@doiabbr{}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{optics}{\gdef\@journal{optics}\gdef\@journalfull{Optics}\gdef\@journalshort{Optics}\gdef\@doiabbr{opt}\gdef\@ISSN{2673-3269}\gdef\@continuouspages{yes}}
\DeclareOption{oral}{\gdef\@journal{oral}\gdef\@journalfull{Oral}\gdef\@journalshort{Oral}\gdef\@doiabbr{oral}\gdef\@ISSN{2673-6373}\gdef\@continuouspages{yes}}
\DeclareOption{organics}{\gdef\@journal{organics}\gdef\@journalfull{Organics}\gdef\@journalshort{Organics}\gdef\@doiabbr{org}\gdef\@ISSN{2673-401X}\gdef\@continuouspages{yes}}
\DeclareOption{organoids}{\gdef\@journal{organoids}\gdef\@journalfull{Organoids}\gdef\@journalshort{Organoids}\gdef\@doiabbr{organoids}\gdef\@ISSN{2674-1172}\gdef\@continuouspages{yes}}
\DeclareOption{osteology}{\gdef\@journal{osteology}\gdef\@journalfull{Osteology}\gdef\@journalshort{Osteology}\gdef\@doiabbr{osteology}\gdef\@ISSN{2673-4036}\gdef\@continuouspages{yes}}
\DeclareOption{oxygen}{\gdef\@journal{oxygen}\gdef\@journalfull{Oxygen}\gdef\@journalshort{Oxygen}\gdef\@doiabbr{oxygen}\gdef\@ISSN{2673-9801}\gdef\@continuouspages{yes}}
\DeclareOption{parasites}{\gdef\@journal{parasites}\gdef\@journalfull{Parasites}\gdef\@journalshort{Parasites}\gdef\@doiabbr{parasites}\gdef\@ISSN{2673-5946}}
\DeclareOption{parasitologia}{\gdef\@journal{parasitologia}\gdef\@journalfull{Parasitologia}\gdef\@journalshort{Parasitologia}\gdef\@doiabbr{parasitologia}\gdef\@ISSN{2673-6772}\gdef\@continuouspages{yes}}
\DeclareOption{particles}{\gdef\@journal{particles}\gdef\@journalfull{Particles}\gdef\@journalshort{Particles}\gdef\@doiabbr{particles}\gdef\@ISSN{2571-712X}\gdef\@continuouspages{yes}}
\DeclareOption{pathogens}{\gdef\@journal{pathogens}\gdef\@journalfull{Pathogens}\gdef\@journalshort{Pathogens}\gdef\@doiabbr{pathogens}\gdef\@ISSN{2076-0817}}
\DeclareOption{pathophysiology}{\gdef\@journal{pathophysiology}\gdef\@journalfull{Pathophysiology}\gdef\@journalshort{Pathophysiology}\gdef\@doiabbr{pathophysiology}\gdef\@ISSN{0928-4680}\gdef\@continuouspages{yes}}
\DeclareOption{pediatrrep}{\gdef\@journal{pediatrrep}\gdef\@journalfull{Pediatric Reports}\gdef\@journalshort{Pediatr. Rep.}\gdef\@doiabbr{pediatric}\gdef\@ISSN{2036-7503}\gdef\@continuouspages{yes}}
\DeclareOption{pets}{\gdef\@journal{pets}\gdef\@journalfull{Pets}\gdef\@journalshort{Pets}\gdef\@doiabbr{pets}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{pharmaceuticals}{\gdef\@journal{pharmaceuticals}\gdef\@journalfull{Pharmaceuticals}\gdef\@journalshort{Pharmaceuticals}\gdef\@doiabbr{ph}\gdef\@ISSN{1424-8247}}
\DeclareOption{pharmaceutics}{\gdef\@journal{pharmaceutics}\gdef\@journalfull{Pharmaceutics}\gdef\@journalshort{Pharmaceutics}\gdef\@doiabbr{pharmaceutics}\gdef\@ISSN{1999-4923}}
\DeclareOption{pharmacoepidemiology}{\gdef\@journal{pharmacoepidemiology}\gdef\@journalfull{Pharmacoepidemiology}\gdef\@journalshort{Pharmacoepidemiology}\gdef\@doiabbr{pharma}\gdef\@ISSN{2813-0618}\gdef\@continuouspages{yes}}
\DeclareOption{pharmacy}{\gdef\@journal{pharmacy}\gdef\@journalfull{Pharmacy}\gdef\@journalshort{Pharmacy}\gdef\@doiabbr{pharmacy}\gdef\@ISSN{2226-4787}}
\DeclareOption{philosophies}{\gdef\@journal{philosophies}\gdef\@journalfull{Philosophies}\gdef\@journalshort{Philosophies}\gdef\@doiabbr{philosophies}\gdef\@ISSN{2409-9287}}
\DeclareOption{photochem}{\gdef\@journal{photochem}\gdef\@journalfull{Photochem}\gdef\@journalshort{Photochem}\gdef\@doiabbr{photochem}\gdef\@ISSN{2673-7256}\gdef\@continuouspages{yes}}
\DeclareOption{photonics}{\gdef\@journal{photonics}\gdef\@journalfull{Photonics}\gdef\@journalshort{Photonics}\gdef\@doiabbr{photonics}\gdef\@ISSN{2304-6732}}
\DeclareOption{phycology}{\gdef\@journal{phycology}\gdef\@journalfull{Phycology}\gdef\@journalshort{Phycology}\gdef\@doiabbr{phycology}\gdef\@ISSN{2673-9410}\gdef\@continuouspages{yes}}
\DeclareOption{physchem}{\gdef\@journal{physchem}\gdef\@journalfull{Physchem}\gdef\@journalshort{Physchem}\gdef\@doiabbr{physchem}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{physics}{\gdef\@journal{physics}\gdef\@journalfull{Physics}\gdef\@journalshort{Physics}\gdef\@doiabbr{physics}\gdef\@ISSN{2624-8174}\gdef\@continuouspages{yes}}
\DeclareOption{physiologia}{\gdef\@journal{physiologia}\gdef\@journalfull{Physiologia}\gdef\@journalshort{Physiologia}\gdef\@doiabbr{physiologia}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{plants}{\gdef\@journal{plants}\gdef\@journalfull{Plants}\gdef\@journalshort{Plants}\gdef\@doiabbr{plants}\gdef\@ISSN{2223-7747}}
\DeclareOption{plasma}{\gdef\@journal{plasma}\gdef\@journalfull{Plasma}\gdef\@journalshort{Plasma}\gdef\@doiabbr{plasma}\gdef\@ISSN{2571-6182}\gdef\@continuouspages{yes}}
\DeclareOption{platforms}{\gdef\@journal{platforms}\gdef\@journalfull{Platforms}\gdef\@journalshort{Platforms}\gdef\@doiabbr{platforms}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{pollutants}{\gdef\@journal{pollutants}\gdef\@journalfull{Pollutants}\gdef\@journalshort{Pollutants}\gdef\@doiabbr{pollutants}\gdef\@ISSN{2673-4672}\gdef\@continuouspages{yes}}
\DeclareOption{polymers}{\gdef\@journal{polymers}\gdef\@journalfull{Polymers}\gdef\@journalshort{Polymers}\gdef\@doiabbr{polym}\gdef\@ISSN{2073-4360}}
\DeclareOption{polysaccharides}{\gdef\@journal{polysaccharides}\gdef\@journalfull{Polysaccharides}\gdef\@journalshort{Polysaccharides}\gdef\@doiabbr{polysaccharides}\gdef\@ISSN{2673-4176}\gdef\@continuouspages{yes}}
\DeclareOption{poultry}{\gdef\@journal{poultry}\gdef\@journalfull{Poultry}\gdef\@journalshort{Poultry}\gdef\@doiabbr{poultry}\gdef\@ISSN{2674-1164}\gdef\@continuouspages{yes}}
\DeclareOption{powders}{\gdef\@journal{powders}\gdef\@journalfull{Powders}\gdef\@journalshort{Powders}\gdef\@doiabbr{powders}\gdef\@ISSN{2674-0516}\gdef\@continuouspages{yes}}
\DeclareOption{preprints}{\gdef\@journal{preprints}\gdef\@journalfull{Preprints}\gdef\@journalshort{Preprints}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{proceedings}{\gdef\@journal{proceedings}\gdef\@journalfull{Proceedings}\gdef\@journalshort{Proceedings}\gdef\@doiabbr{proceedings}\gdef\@ISSN{2504-3900}}
\DeclareOption{processes}{\gdef\@journal{processes}\gdef\@journalfull{Processes}\gdef\@journalshort{Processes}\gdef\@doiabbr{pr}\gdef\@ISSN{2227-9717}}
\DeclareOption{prosthesis}{\gdef\@journal{prosthesis}\gdef\@journalfull{Prosthesis}\gdef\@journalshort{Prosthesis}\gdef\@doiabbr{prosthesis}\gdef\@ISSN{2673-1592}\gdef\@continuouspages{yes}}
\DeclareOption{proteomes}{\gdef\@journal{proteomes}\gdef\@journalfull{Proteomes}\gdef\@journalshort{Proteomes}\gdef\@doiabbr{proteomes}\gdef\@ISSN{2227-7382}}
\DeclareOption{psf}{\gdef\@journal{psf}\gdef\@journalfull{Physical Sciences Forum}\gdef\@journalshort{Phys. Sci. Forum}\gdef\@doiabbr{psf}\gdef\@ISSN{2673-9984}}
%\DeclareOption{psych}{\gdef\@journal{psych}\gdef\@journalfull{Psych}\gdef\@journalshort{Psych}\gdef\@doiabbr{psych}\gdef\@ISSN{2624-8611}\gdef\@continuouspages{yes}} % Have changed to psycholint
\DeclareOption{psycholint}{\gdef\@journal{psycholint}\gdef\@journalfull{Psychology International}\gdef\@journalshort{Psychol. Int.}\gdef\@doiabbr{psycholint}\gdef\@ISSN{2813-9844}\gdef\@continuouspages{yes}}
\DeclareOption{psychiatryint}{\gdef\@journal{psychiatryint}\gdef\@journalfull{Psychiatry International}\gdef\@journalshort{Psychiatry Int.}\gdef\@doiabbr{psychiatryint}\gdef\@ISSN{2673-5318}\gdef\@continuouspages{yes}}
\DeclareOption{psychoactives}{\gdef\@journal{psychoactives}\gdef\@journalfull{Psychoactives}\gdef\@journalshort{Psychoactives}\gdef\@doiabbr{psychoactives}\gdef\@ISSN{2813-1851}\gdef\@continuouspages{yes}}
\DeclareOption{publications}{\gdef\@journal{publications}\gdef\@journalfull{Publications}\gdef\@journalshort{Publications}\gdef\@doiabbr{publications}\gdef\@ISSN{2304-6775}}
\DeclareOption{purification}{\gdef\@journal{purification}\gdef\@journalfull{Purification}\gdef\@journalshort{Purification}\gdef\@doiabbr{purification}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{quantumrep}{\gdef\@journal{quantumrep}\gdef\@journalfull{Quantum Reports}\gdef\@journalshort{Quantum Rep.}\gdef\@doiabbr{quantum}\gdef\@ISSN{2624-960X}\gdef\@continuouspages{yes}}
\DeclareOption{quaternary}{\gdef\@journal{quaternary}\gdef\@journalfull{Quaternary}\gdef\@journalshort{Quaternary}\gdef\@doiabbr{quat}\gdef\@ISSN{2571-550X}}
\DeclareOption{qubs}{\gdef\@journal{qubs}\gdef\@journalfull{Quantum Beam Science}\gdef\@journalshort{Quantum Beam Sci.}\gdef\@doiabbr{qubs}\gdef\@ISSN{2412-382X}}
\DeclareOption{radiation}{\gdef\@journal{radiation}\gdef\@journalfull{Radiation}\gdef\@journalshort{Radiation}\gdef\@doiabbr{radiation}\gdef\@ISSN{2673-592X}\gdef\@continuouspages{yes}}
\DeclareOption{reactions}{\gdef\@journal{reactions}\gdef\@journalfull{Reactions}\gdef\@journalshort{Reactions}\gdef\@doiabbr{reactions}\gdef\@ISSN{2624-781X}\gdef\@continuouspages{yes}}
\DeclareOption{realestate}{\gdef\@journal{realestate}\gdef\@journalfull{Real Estate}\gdef\@journalshort{Real Estate}\gdef\@doiabbr{realestate}\gdef\@ISSN{2813-8090}\gdef\@continuouspages{yes}}
\DeclareOption{receptors}{\gdef\@journal{receptors}\gdef\@journalfull{Receptors}\gdef\@journalshort{Receptors}\gdef\@doiabbr{receptors}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{recycling}{\gdef\@journal{recycling}\gdef\@journalfull{Recycling}\gdef\@journalshort{Recycling}\gdef\@doiabbr{recycling}\gdef\@ISSN{2313-4321}}
\DeclareOption{regeneration}{\gdef\@journal{regeneration}\gdef\@journalfull{Regeneration}\gdef\@journalshort{Regeneration}\gdef\@doiabbr{regeneration}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{religions}{\gdef\@journal{religions}\gdef\@journalfull{Religions}\gdef\@journalshort{Religions}\gdef\@doiabbr{rel}\gdef\@ISSN{2077-1444}}
\DeclareOption{remotesensing}{\gdef\@journal{remotesensing}\gdef\@journalfull{Remote Sensing}\gdef\@journalshort{Remote Sens.}\gdef\@doiabbr{rs}\gdef\@ISSN{2072-4292}}
\DeclareOption{reports}{\gdef\@journal{reports}\gdef\@journalfull{Reports}\gdef\@journalshort{Reports}\gdef\@doiabbr{reports}\gdef\@ISSN{2571-841X}}
\DeclareOption{reprodmed}{\gdef\@journal{reprodmed}\gdef\@journalfull{Reproductive Medicine}\gdef\@journalshort{Reprod. Med.}\gdef\@doiabbr{reprodmed}\gdef\@ISSN{2673-3897}\gdef\@continuouspages{yes}}
\DeclareOption{resources}{\gdef\@journal{resources}\gdef\@journalfull{Resources}\gdef\@journalshort{Resources}\gdef\@doiabbr{resources}\gdef\@ISSN{2079-9276}}
\DeclareOption{rheumato}{\gdef\@journal{rheumato}\gdef\@journalfull{Rheumato}\gdef\@journalshort{Rheumato}\gdef\@doiabbr{rheumato}\gdef\@ISSN{2674-0621}\gdef\@continuouspages{yes}}
\DeclareOption{risks}{\gdef\@journal{risks}\gdef\@journalfull{Risks}\gdef\@journalshort{Risks}\gdef\@doiabbr{risks}\gdef\@ISSN{2227-9091}}
\DeclareOption{robotics}{\gdef\@journal{robotics}\gdef\@journalfull{Robotics}\gdef\@journalshort{Robotics}\gdef\@doiabbr{robotics}\gdef\@ISSN{2218-6581}}
\DeclareOption{ruminants}{\gdef\@journal{ruminants}\gdef\@journalfull{Ruminants}\gdef\@journalshort{Ruminants}\gdef\@doiabbr{ruminants}\gdef\@ISSN{2673-933X}\gdef\@continuouspages{yes}}
\DeclareOption{safety}{\gdef\@journal{safety}\gdef\@journalfull{Safety}\gdef\@journalshort{Safety}\gdef\@doiabbr{safety}\gdef\@ISSN{2313-576X}}
\DeclareOption{sci}{\gdef\@journal{sci}\gdef\@journalfull{Sci}\gdef\@journalshort{Sci}\gdef\@doiabbr{sci}\gdef\@ISSN{2413-4155}}
\DeclareOption{scipharm}{\gdef\@journal{scipharm}\gdef\@journalfull{Scientia Pharmaceutica}\gdef\@journalshort{Sci. Pharm.}\gdef\@doiabbr{scipharm}\gdef\@ISSN{2218-0532}}
\DeclareOption{sclerosis}{\gdef\@journal{sclerosis}\gdef\@journalfull{Sclerosis}\gdef\@journalshort{Sclerosis}\gdef\@doiabbr{sclerosis}\gdef\@ISSN{2813-3064}\gdef\@continuouspages{yes}}
\DeclareOption{seeds}{\gdef\@journal{seeds}\gdef\@journalfull{Seeds}\gdef\@journalshort{Seeds}\gdef\@doiabbr{seeds}\gdef\@ISSN{2674-1024}\gdef\@continuouspages{yes}}
\DeclareOption{sensors}{\gdef\@journal{sensors}\gdef\@journalfull{Sensors}\gdef\@journalshort{Sensors}\gdef\@doiabbr{s}\gdef\@ISSN{1424-8220}}
\DeclareOption{separations}{\gdef\@journal{separations}\gdef\@journalfull{Separations}\gdef\@journalshort{Separations}\gdef\@doiabbr{separations}\gdef\@ISSN{2297-8739}}
\DeclareOption{sexes}{\gdef\@journal{sexes}\gdef\@journalfull{Sexes}\gdef\@journalshort{Sexes}\gdef\@doiabbr{sexes}\gdef\@ISSN{2411-5118}\gdef\@continuouspages{yes}}
\DeclareOption{signals}{\gdef\@journal{signals}\gdef\@journalfull{Signals}\gdef\@journalshort{Signals}\gdef\@doiabbr{signals}\gdef\@ISSN{2624-6120}\gdef\@continuouspages{yes}}
\DeclareOption{sinusitis}{\gdef\@journal{sinusitis}\gdef\@journalfull{Sinusitis}\gdef\@journalshort{Sinusitis}\gdef\@doiabbr{sinusitis}\gdef\@ISSN{2309-107X}\gdef\@continuouspages{yes}}
\DeclareOption{siuj}{\gdef\@journal{siuj}\gdef\@journalfull{Soci\'{e}t\'{e} Internationale d'Urologie Journal}\gdef\@journalshort{Soc. Int. Urol. J.}\gdef\@doiabbr{siuj}\gdef\@ISSN{2563-6499}\gdef\@continuouspages{yes}}
\DeclareOption{skins}{\gdef\@journal{skins}\gdef\@journalfull{Skins}\gdef\@journalshort{Skins}\gdef\@doiabbr{skins}\gdef\@ISSN{}}
\DeclareOption{smartcities}{\gdef\@journal{smartcities}\gdef\@journalfull{Smart Cities}\gdef\@journalshort{Smart Cities}\gdef\@doiabbr{smartcities}\gdef\@ISSN{2624-6511}\gdef\@continuouspages{yes}}
\DeclareOption{sna}{\gdef\@journal{sna}\gdef\@journalfull{Sinusitis and Asthma}\gdef\@journalshort{Sinusitis Asthma}\gdef\@doiabbr{sna}\gdef\@ISSN{2624-7003}}
\DeclareOption{societies}{\gdef\@journal{societies}\gdef\@journalfull{Societies}\gdef\@journalshort{Societies}\gdef\@doiabbr{soc}\gdef\@ISSN{2075-4698}}
\DeclareOption{socsci}{\gdef\@journal{socsci}\gdef\@journalfull{Social Sciences}\gdef\@journalshort{Soc. Sci.}\gdef\@doiabbr{socsci}\gdef\@ISSN{2076-0760}}
\DeclareOption{software}{\gdef\@journal{software}\gdef\@journalfull{Software}\gdef\@journalshort{Software}\gdef\@doiabbr{software}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{soilsystems}{\gdef\@journal{soilsystems}\gdef\@journalfull{Soil Systems}\gdef\@journalshort{Soil Syst.}\gdef\@doiabbr{soilsystems}\gdef\@ISSN{2571-8789}}
\DeclareOption{solar}{\gdef\@journal{solar}\gdef\@journalfull{Solar}\gdef\@journalshort{Solar}\gdef\@doiabbr{solar}\gdef\@ISSN{2673-9941}\gdef\@continuouspages{yes}}
\DeclareOption{solids}{\gdef\@journal{solids}\gdef\@journalfull{Solids}\gdef\@journalshort{Solids}\gdef\@doiabbr{solids}\gdef\@ISSN{2673-6497}\gdef\@continuouspages{yes}}
\DeclareOption{spectroscj}{\gdef\@journal{spectroscj}\gdef\@journalfull{Spectroscopy Journal}\gdef\@journalshort{Spectrosc. J.}\gdef\@doiabbr{spectroscj}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{sports}{\gdef\@journal{sports}\gdef\@journalfull{Sports}\gdef\@journalshort{Sports}\gdef\@doiabbr{sports}\gdef\@ISSN{2075-4663}}
\DeclareOption{standards}{\gdef\@journal{standards}\gdef\@journalfull{Standards}\gdef\@journalshort{Standards}\gdef\@doiabbr{standards}\gdef\@ISSN{2305-6703}\gdef\@continuouspages{yes}}
\DeclareOption{stats}{\gdef\@journal{stats}\gdef\@journalfull{Stats}\gdef\@journalshort{Stats}\gdef\@doiabbr{stats}\gdef\@ISSN{2571-905X}\gdef\@continuouspages{yes}}
\DeclareOption{std}{\gdef\@journal{std}\gdef\@journalfull{Surgical Techniques Development}\gdef\@journalshort{Surg. Tech. Dev.}\gdef\@doiabbr{std}\gdef\@ISSN{2038-9582}\gdef\@continuouspages{yes}}
\DeclareOption{stresses}{\gdef\@journal{stresses}\gdef\@journalfull{Stresses}\gdef\@journalshort{Stresses}\gdef\@doiabbr{stresses}\gdef\@ISSN{2673-7140}\gdef\@continuouspages{yes}}
\DeclareOption{surfaces}{\gdef\@journal{surfaces}\gdef\@journalfull{Surfaces}\gdef\@journalshort{Surfaces}\gdef\@doiabbr{surfaces}\gdef\@ISSN{2571-9637}\gdef\@continuouspages{yes}}
\DeclareOption{surgeries}{\gdef\@journal{surgeries}\gdef\@journalfull{Surgeries}\gdef\@journalshort{Surgeries}\gdef\@doiabbr{surgeries}\gdef\@ISSN{2017-2017}\gdef\@continuouspages{yes}}
\DeclareOption{suschem}{\gdef\@journal{suschem}\gdef\@journalfull{Sustainable Chemistry}\gdef\@journalshort{Sustain. Chem.}\gdef\@doiabbr{suschem}\gdef\@ISSN{2673-4079}\gdef\@continuouspages{yes}}
\DeclareOption{sustainability}{\gdef\@journal{sustainability}\gdef\@journalfull{Sustainability}\gdef\@journalshort{Sustainability}\gdef\@doiabbr{su}\gdef\@ISSN{2071-1050}}
\DeclareOption{symmetry}{\gdef\@journal{symmetry}\gdef\@journalfull{Symmetry}\gdef\@journalshort{Symmetry}\gdef\@doiabbr{sym}\gdef\@ISSN{2073-8994}}
\DeclareOption{synbio}{\gdef\@journal{synbio}\gdef\@journalfull{SynBio}\gdef\@journalshort{SynBio}\gdef\@doiabbr{synbio}\gdef\@ISSN{2674-0583}\gdef\@continuouspages{yes}}
\DeclareOption{systems}{\gdef\@journal{systems}\gdef\@journalfull{Systems}\gdef\@journalshort{Systems}\gdef\@doiabbr{systems}\gdef\@ISSN{2079-8954}}
\DeclareOption{targets}{\gdef\@journal{targets}\gdef\@journalfull{Targets}\gdef\@journalshort{Targets}\gdef\@doiabbr{targets}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{taxonomy}{\gdef\@journal{taxonomy}\gdef\@journalfull{Taxonomy}\gdef\@journalshort{Taxonomy}\gdef\@doiabbr{taxonomy}\gdef\@ISSN{2673-6500}\gdef\@continuouspages{yes}}
\DeclareOption{technologies}{\gdef\@journal{technologies}\gdef\@journalfull{Technologies}\gdef\@journalshort{Technologies}\gdef\@doiabbr{technologies}\gdef\@ISSN{2227-7080}}
\DeclareOption{telecom}{\gdef\@journal{telecom}\gdef\@journalfull{Telecom}\gdef\@journalshort{Telecom}\gdef\@doiabbr{telecom}\gdef\@ISSN{2673-4001}\gdef\@continuouspages{yes}}
\DeclareOption{test}{\gdef\@journal{test}\gdef\@journalfull{Test}\gdef\@journalshort{Test}\gdef\@doiabbr{}\gdef\@ISSN{}}
\DeclareOption{textiles}{\gdef\@journal{textiles}\gdef\@journalfull{Textiles}\gdef\@journalshort{Textiles}\gdef\@doiabbr{textiles}\gdef\@ISSN{2673-7248}\gdef\@continuouspages{yes}}
\DeclareOption{thalassrep}{\gdef\@journal{thalassrep}\gdef\@journalfull{Thalassemia Reports}\gdef\@journalshort{Thalass. Rep.}\gdef\@doiabbr{thalassrep}\gdef\@ISSN{2039-4365}\gdef\@continuouspages{yes}}
\DeclareOption{therapeutics}{\gdef\@journal{therapeutics}\gdef\@journalfull{Therapeutics}\gdef\@journalshort{Therapeutics}\gdef\@doiabbr{therapeutics}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{thermo}{\gdef\@journal{thermo}\gdef\@journalfull{Thermo}\gdef\@journalshort{Thermo}\gdef\@doiabbr{thermo}\gdef\@ISSN{2673-7264}\gdef\@continuouspages{yes}}
\DeclareOption{timespace}{\gdef\@journal{timespace}\gdef\@journalfull{Time and Space}\gdef\@journalshort{Time Space}\gdef\@doiabbr{timespace}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{tomography}{\gdef\@journal{tomography}\gdef\@journalfull{Tomography}\gdef\@journalshort{Tomography}\gdef\@doiabbr{tomography}\gdef\@ISSN{2379-139X}\gdef\@continuouspages{yes}}
\DeclareOption{tourismhosp}{\gdef\@journal{tourismhosp}\gdef\@journalfull{Tourism and Hospitality}\gdef\@journalshort{Tour. Hosp.}\gdef\@doiabbr{tourhosp}\gdef\@ISSN{2673-5768}\gdef\@continuouspages{yes}}
\DeclareOption{toxics}{\gdef\@journal{toxics}\gdef\@journalfull{Toxics}\gdef\@journalshort{Toxics}\gdef\@doiabbr{toxics}\gdef\@ISSN{2305-6304}}
\DeclareOption{toxins}{\gdef\@journal{toxins}\gdef\@journalfull{Toxins}\gdef\@journalshort{Toxins}\gdef\@doiabbr{toxins}\gdef\@ISSN{2072-6651}}
\DeclareOption{transplantology}{\gdef\@journal{transplantology}\gdef\@journalfull{Transplantology}\gdef\@journalshort{Transplantology}\gdef\@doiabbr{transplantology}\gdef\@ISSN{2673-3943}\gdef\@continuouspages{yes}}
\DeclareOption{transportation}{\gdef\@journal{transportation}\gdef\@journalfull{Transportation}\gdef\@journalshort{Transportation}\gdef\@doiabbr{transportation}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{traumacare}{\gdef\@journal{traumacare}\gdef\@journalfull{Trauma Care}\gdef\@journalshort{Trauma Care}\gdef\@doiabbr{traumacare}\gdef\@ISSN{2673-866X}\gdef\@continuouspages{yes}}
\DeclareOption{traumas}{\gdef\@journal{traumas}\gdef\@journalfull{Traumas}\gdef\@journalshort{Traumas}\gdef\@doiabbr{traumas}\gdef\@ISSN{2673-7477}\gdef\@continuouspages{yes}}
\DeclareOption{tropicalmed}{\gdef\@journal{tropicalmed}\gdef\@journalfull{Tropical Medicine and Infectious Disease}\gdef\@journalshort{Trop. Med. Infect. Dis.}\gdef\@doiabbr{tropicalmed}\gdef\@ISSN{2414-6366}}
\DeclareOption{universe}{\gdef\@journal{universe}\gdef\@journalfull{Universe}\gdef\@journalshort{Universe}\gdef\@doiabbr{universe}\gdef\@ISSN{2218-1997}}
\DeclareOption{urbansci}{\gdef\@journal{urbansci}\gdef\@journalfull{Urban Science}\gdef\@journalshort{Urban Sci.}\gdef\@doiabbr{urbansci}\gdef\@ISSN{2413-8851}}
\DeclareOption{uro}{\gdef\@journal{uro}\gdef\@journalfull{Uro}\gdef\@journalshort{Uro}\gdef\@doiabbr{uro}\gdef\@ISSN{2673-4397}\gdef\@continuouspages{yes}}
\DeclareOption{vaccines}{\gdef\@journal{vaccines}\gdef\@journalfull{Vaccines}\gdef\@journalshort{Vaccines}\gdef\@doiabbr{vaccines}\gdef\@ISSN{2076-393X}}
\DeclareOption{vehicles}{\gdef\@journal{vehicles}\gdef\@journalfull{Vehicles}\gdef\@journalshort{Vehicles}\gdef\@doiabbr{vehicles}\gdef\@ISSN{2624-8921}\gdef\@continuouspages{yes}}
\DeclareOption{venereology}{\gdef\@journal{venereology}\gdef\@journalfull{Venereology}\gdef\@journalshort{Venereology}\gdef\@doiabbr{venereology}\gdef\@ISSN{2674-0710}\gdef\@continuouspages{yes}}
\DeclareOption{vetsci}{\gdef\@journal{vetsci}\gdef\@journalfull{Veterinary Sciences}\gdef\@journalshort{Vet. Sci.}\gdef\@doiabbr{vetsci}\gdef\@ISSN{2306-7381}}
\DeclareOption{vibration}{\gdef\@journal{vibration}\gdef\@journalfull{Vibration}\gdef\@journalshort{Vibration}\gdef\@doiabbr{vibration}\gdef\@ISSN{2571-631X}\gdef\@continuouspages{yes}}
\DeclareOption{virtualworlds}{\gdef\@journal{virtualworlds}\gdef\@journalfull{Virtual Worlds}\gdef\@journalshort{Virtual Worlds}\gdef\@doiabbr{virtualworlds}\gdef\@ISSN{}\gdef\@continuouspages{yes}}
\DeclareOption{viruses}{\gdef\@journal{viruses}\gdef\@journalfull{Viruses}\gdef\@journalshort{Viruses}\gdef\@doiabbr{v}\gdef\@ISSN{1999-4915}}
\DeclareOption{vision}{\gdef\@journal{vision}\gdef\@journalfull{Vision}\gdef\@journalshort{Vision}\gdef\@doiabbr{vision}\gdef\@ISSN{2411-5150}}
\DeclareOption{waste}{\gdef\@journal{waste}\gdef\@journalfull{Waste}\gdef\@journalshort{Waste}\gdef\@doiabbr{waste}\gdef\@ISSN{2813-0391}\gdef\@continuouspages{yes}}
\DeclareOption{water}{\gdef\@journal{water}\gdef\@journalfull{Water}\gdef\@journalshort{Water}\gdef\@doiabbr{w}\gdef\@ISSN{2073-4441}}
\DeclareOption{wem}{\gdef\@journal{wem}\gdef\@journalfull{Wildlife Ecology and Management}\gdef\@journalshort{Wildl. Ecol. Manag.}\gdef\@doiabbr{}\gdef\@ISSN{1234-4321}}
\DeclareOption{wevj}{\gdef\@journal{wevj}\gdef\@journalfull{World Electric Vehicle Journal}\gdef\@journalshort{World Electr. Veh. J.}\gdef\@doiabbr{wevj}\gdef\@ISSN{2032-6653}}
\DeclareOption{wind}{\gdef\@journal{wind}\gdef\@journalfull{Wind}\gdef\@journalshort{Wind}\gdef\@doiabbr{wind}\gdef\@ISSN{2674-032X}\gdef\@continuouspages{yes}}
\DeclareOption{women}{\gdef\@journal{women}\gdef\@journalfull{Women}\gdef\@journalshort{Women}\gdef\@doiabbr{women}\gdef\@ISSN{2673-4184}\gdef\@continuouspages{yes}}
\DeclareOption{world}{\gdef\@journal{world}\gdef\@journalfull{World}\gdef\@journalshort{World}\gdef\@doiabbr{world}\gdef\@ISSN{2673-4060}\gdef\@continuouspages{yes}}
\DeclareOption{youth}{\gdef\@journal{youth}\gdef\@journalfull{Youth}\gdef\@journalshort{Youth}\gdef\@doiabbr{youth}\gdef\@ISSN{2673-995X}\gdef\@continuouspages{yes}}
\DeclareOption{zoonoticdis}{\gdef\@journal{zoonoticdis}\gdef\@journalfull{Zoonotic Diseases}\gdef\@journalshort{Zoonotic Dis.}\gdef\@doiabbr{zoonoticdis}\gdef\@ISSN{2813-0227}\gdef\@continuouspages{yes}}


==> sections/010_intro.tex <==
\section{Introduction}
\label{sec:intro}

Deep neural networks have established themselves as the primary algorithmic solution for a wide array of real-world applications. However, the computational and memory requirements of DNNs are considerable, leading to notable latency and power consumption during both training and inference processes.

To meet the rapidly increasing demand for algorithmic capabilities in embedded systems, such as autonomous vehicles, drones, and medical devices, prior research has suggested various techniques for reducing these devices' power and energy consumption.
Some of the techniques already deployed in different systems are matrix compression \cite{Lebedev2015SpeedingupCN, Ullrich2017SoftWF,9206968,JMLR:v22:20-1374}, pruning \cite{Han2015LearningBW, Wen2016LearningSS}, hardware-aware neural architecture search \cite{Liu2019DARTSDA, Wu2019FBNetHE, Cai2019ProxylessNASDN}, and quantization \cite{zhou2016dorefa,hubara2017,Choi2018PACTPC}.

Quantization is a promising and straightforward technique to accelerate neural network architecture because it reduces the model's memory footprint and the computation complexity by a large factor.

The standard metric to evaluate a quantized model's computational complexity is the number of multiply-accumulate (MAC) operations or bit operations (BOPS) it demands. Both do not consider other factors such as communication complexity \cite{9177369}, memory utilization, and inter-layer relations.
Using ultra-low bit quantization does not, therefore, consistently improve the chip's overall performance due to communication and memory boundaries \cite{su13020717}.

To this end, recent developments in industry \cite{apple,nvidia} and academia \cite{samajdar2020systematic,Sharma2018BitFB} introduced  support for various precision matrix multiplications, leading to a new line of work focusing on Mixed-Precision (MP) quantization \cite{Wang2018HAQHA,Dong2019HAWQHA,Sun2022FILMQNNEF}, that is, assigning different bandwidth to each matrix (i.e., weights and activations).

\begin{figure}
	\centering
% 	\vspace{-1.3cm}
	\includegraphics[width=1.\textwidth]{figures/RN50.pdf} 
	\vspace{-0.3cm}
	\caption{ResNet-50 quantized models on a latency-accuracy plane. Circles are mixed-precision quantization and triangles are uniform quantization.
	Our models achieve a better Pareto curve of dominant solutions in the two-dimensional plane for ultra-low precision.}
	\label{fig:resnet50}
\end{figure}

MP quantization methods focuses on either finding the an optimal solution by estimation of the loss manifold of a full-precision model and asses what layers would cause the least steepest change to the local minima the model reached at one quantization step \cite{Dong2019HAWQHA,Wang2018HAQHA}. In this work, we argue that when quantizing a model \textit{during} the training process, the  minima on this loss manifold could be very different. This realization lead us to the conclusion that the quantization should be looked at as a process, and the optimal step depend on the intermediate state of the model and not on a final form. This way, an intermediate quantized model would be easier to train and the quantization loss would be lower so the trajectory to the final quantized model is smoother.

Hardware-aware methodologies, sometimes coupled with Neural Architectural Search (NAS), has shown promising progress in the field of hardware-aware models. Current work \cite{Wu2019FBNetHE,Cai2019ProxylessNASDN} directly measure signals from the hardware simulator. Nevertheless, to incorporate hardware constraints into the loss, they neglect the dependencies between layers, that is, the latency per layer per precision is a fixed number. This assumption is inaccurate in cases where the memory utilization is high because the communication boundary accedes to the computational one. NAS can provide a solution that is better tailored to the task, Even so, the search space is commonly huge, and the cost of training \cite{Sun2019AnEL} and the carbon footprint \cite{Strubell2019EnergyAP} are high.

Our solution, Automatic Mixed-Precision Quantization for Edge Devices (dubbed \methodname), is an algorithmic framework that chooses mixed-precision bit allocation per layer by looking at reduced precision as a Markov Decision Process (MDP), using signals directly from the hardware. 
The procedure is simple to use, not bounded to a specific HW design and easily fine-tuned by the user to find a good balance between performance and resource consumption.

This paper makes the following contributions:

\begin{itemize}
    \item A novel framework for mixed-precision quantization for DNNs that look at reduced precision as a markov process.
    \item A quality score that represents the accuracy--latency trade-off w.r.t. the hardware constraint. This allows us to create custom-fitted solutions for a range of device-specific hardware constraints via direct hardware signals to the training procedure.
    \item Extensive experiments conducted on different hardware setups with different models on standard image classification benchmarks (CIFAR100, ImageNet). These outperform previous methods in terms of the accuracy--latency trade-off.
    \item A proposed modular framework, i.e., the sampling method, hardware properties, accelerator simulator, and neural network architecture are all independent modules, making it applicable to any given case.  
\end{itemize}



      

==> sections/020_related.tex <==
\section{Materials}%preliminary and Related Work}
\label{sec:related}
\subsection*{Multi-objective optimization}
\label{subsec:mul obj opt}
In a simple learning paradigm, the optimization process attempts to minimize an objective function; The example in this work is of classification model, minimizing the cross-entropy loss, denoted by $\mathcal{L}_{CE}$.

Multi-objective problems can have both positively correlated objectives as well as negatively correlated objectives (also known as conflicting objectives or adversary objectives).
The problem we aim to solve in this paper is the accuracy--latency trade-off of quantized model, in which one objective is minimizing $\mathcal{L}_{CE}$ while the other is minimizing the latency, denoted by $\mathcal{L}_{lat}$. This idea can be extended to other hardware objectives (such as model size or power consumption); however, these typically correlated to $\mathcal{L}_{lat}$ and kept beyond of the scope of this work.  

Both objectives are conflicting because quantizing our model to lower representation aim to reduces latency with the cost of increased quantization error.
Due to these conflicting objectives, multi-objective optimization problems are known to lack optimal solutions w.r.t. all of the objectives \cite{10.1162/evco.1994.2.3.221}. Typically, there are many optimal (or suboptimal) solutions because one is not comparable to the other.
Solution $\textbf{A}$ dominates solution $\textbf{B}$ ($\textbf{A} \prec \textbf{B}$) if all objective values of $\textbf{A}$ are better than or equal to the respective objective value of $\textbf{B}$.
Dominant solutions define a Pareto-optimal curve in the objective's plane.
To solve multi-objective optimization, it is very common to use single-objective approaches or a Pareto approach.

A \textbf{single-objective approach} aggregates the objectives into one term, where the basic aggregation method is the weighted sum vector \cite{kdeb01}, we denoted by $\alpha$, which encodes the user's priorities over the different objectives. This method is very common when training a DNN, but has the following drawbacks:
\begin{itemize}
\item The weighted sum vector $\alpha$ must be determined beforehand, and requires a grid search or meta-learning, both of which can be costly and hard to converge.
\item Not all objectives can be optimized via the same optimization scheme. For example, a gradient-based optimizer cannot be used when only some of the objectives are differentiable.
\end{itemize}

A \textbf{Pareto approach} is based on sampling methods and finding the Pareto curve by adopting only dominant solutions.
The main drawback of this approach in the perspective of a quantization scheme is the computational cost. Each sample needs to first quantize a neural network and train it, before it can evaluate the objectives.




\section{Literature review}
\subsection*{Quantized neural networks}
Quantization is one of the most efficient and commonly used techniques for the acceleration and compression of models. Generally, quantization procedures can be categorized into Post-Training Quantization (PTQ) and Quantization-Aware Training (QAT). 
\begin{itemize}
    \item \textbf{PTQ} uses a small calibration set to obtain the optimal quantization parameters without the need or capability to use the entire dataset.
    \item \textbf{QAT} conducts the quantization during the training process and thus uses the entire training corpus.
   \end{itemize}
QAT is more appealing when quantizing a model into ultra-low precision because the network is trained to withhold quantization noise \cite{Li2017TrainingQN}.
Because we are focusing on ultra-low precision, we use the QAT technique for this work. 

Homogeneous quantization quantizes both weights and activations using the same bitwidth throughout the network, scaling from 32-bit to as low as binary \cite{Hubara2016BinarizedNN,Rozen2022BimodalDB}. \cite{Zhang2018LQNetsLQ} proposes a learnable quantizer with a basis vector that is adaptive to the weights and activations. \cite{Choi2018PACTPC,Baskin2021NICENI} presents a clipping method that automatically optimizes the quantization scales during model training. In \cite{Esser2020LSQ}, a non-uniform step-size is learned as a model parameter so that it becomes more sensitive to the quantization transition points. \cite{Han2021ImprovingLN} takes this method a step further and proposes a weight regularization algorithm that encourages a sharp distribution for each quantization bin and encourages it to be as close to the target quantized value as possible. \cite{Gong2019DifferentiableSQ} employs a series of hyperbolic tangent functions to approach the staircase function for low-bit quantization gradually.

Recent research, however, has shows that different layers in a DNN model contribute to the performance differently and contain different redundancies. Therefore, the notion of a mixed-precision quantization scheme that assigns a different precision bitwidth to each layer of the DNN can offer better accuracy while compressing the model even further. Nevertheless, determining each layer's precision is quite challenging because of the large search space. In \cite{Zur2019TowardsLO}, NAS is used for allocating bitwidth by employing BOPS in the cost function. HAQ \cite{Wang2018HAQHA} leverages reinforcement learning to determine the quantization policy layer-wise. Additionally, it takes the hardware accelerator's feedback into account in the architecture design, attaining an optimized solution for deterministic constraints. It fails, However, to find a solution that stochastically reduces latency and power consumption. FBNET \cite{Wu2019FBNetHE} combines all possible design choices into a stochastic super-net and approximates the optimal scheme via sampling. These search methods can require a large quantity of computational resources that scale up quickly with the number of layers.

Therefore, other works attempt to allocate the bitwidth using different methods. \cite{Zhao2021DistributionawareAM} use the first-order Taylor expansion to evaluate the loss sensitivity due to quantization of each channel, and then adjust the bitwidth channel-wise. \cite{Yang2021BSQEB} consider each layer's bitwidth as an independent trainable parameter. \cite{Yang2021FracBitsMP} allocates differentiable bitwidths to layers, which consequently offers smooth transitions between neighboring quantization bit levels, all while meeting a target computational constraint. HAWQ \cite{Dong2019HAWQHA,Dong2020HAWQV2HA} applies mixed-precision quantization using the Hessian information. Power iteration is adopted to compute the top Hessian eigenvalue, which is used to determine which layers are more prone to quantization. It relies on a proxy signal that assumes that all devices benefit from a higher compression rate and a lower number of operations, and does not consider the specific hardware design. \cite{Chen2021TowardsMQ} also uses the Hessian trace and formulates the mixed-precision quantization as a discrete constrained optimization problem solved by a greedy search algorithm. \cite{Zhang2021DifferentiableDQ} differentially learns quantization parameters for each layer, including bitwidth, quantization level, and dynamic range. 
FILM-QNN \cite{Sun2022FILMQNNEF} investigates mixed precision quantization in the layer scope. This means that each layer's parameters have a different precision. While this has the benefit of being even more efficient, the metadata for which parameters send to which multiply and accumulate (MAC) unit is not feasible in most current hardware architectures.
% \TR{BIT MIXER} propose to train a metaquantized network which during test time can switch to any quantization level for any layer in the network - not relevant to us

The quantization can also be performed in two different ways. Works such as \cite{Esser2020LSQ,Gong2019DifferentiableSQ,Yang2021BSQEB,Wang2018HAQHA,Dong2020HAWQV2HA} perform uniform quantization in which the width of the quantization bins is a single parameter. A more complex non-uniform quantization allows different bin widths, which reduces the quantization error \cite{Zhang2018LQNetsLQ,Zhao2021DistributionawareAM}. 

To perform a standard MAC operation in a fixed-point representation on a given hardware, all of the data (weights and activations) must be equally scaled. This means that, when implementing non-uniform quantization, a lookup table to a higher representation is required. While the communication costs are reduced, the computational and area costs of non-uniform quantization are very high and inefficient.

==> sections/030_method.tex <==
\section{Method}
\label{sec:method}
This section introduces our proposed technique for mixed-precision quantization. It leverages the strengths of both approaches described in Section~\ref{subsec:mul obj opt}. We achieve this by first combining the desired properties of the model into a single, unified objective function. Then, we employ the Pareto optimization approach to efficiently sample solutions that achieve a desirable trade-off between these properties.
We define the problem (Section \ref{method:problem def}), describe our perspective of the quantization process of neural networks (Section \ref{method" MMC}), following which we describe our MP quantizer (Section \ref{method: quantizer}) and our MP simulator (Section \ref{method: sim}). Finally, we introduce the technique of \methodname{} (Section \ref{method: AMED}).


\subsection{Problem definition}
\label{method:problem def}
The DNN architecture parameters grouped into $\bb{N}$ layers are denoted by ${\theta}$. The bit-allocation vector is denoted by $\bb{A} \in \mathbb{M}^{\bb{N}}$, where $\mathbb{M}$ is the number of possible bit allocations. Additionally, a quantized set of model parameters is denoted by ${\theta_A}$.
$\bb{A}$ is a temporal vector, denoted by $\bb{A}_t$ at time $t$, and the $l$-th layer bitwidth at time $t$ is denoted by $\bb{A}^l_t$. 

\begin{figure}
	\centering
% 	\vspace{-1.3cm}
	\includegraphics[width=1.\textwidth]{figures/network.drawio.pdf} 
	\vspace{-0.3cm}
	\caption{A diagram of DNN architecture activation maps.}
	\label{fig:diagram}
\end{figure}



Due to the dependence on specific accelerator properties, a differentiable form of the hardware objective (e.g., latency) cannot be directly measured in advance. This renders traditional optimization techniques relying on gradient descent inapplicable. Furthermore, the non-i.i.d. nature of latency across layers adds another layer of complexity. Quantization choices for one layer (e.g., $\bb{A}^{l-1}$ ) can influence the cache behavior of subsequent layers (e.g., l), leading to unpredictable changes in overall latency. This makes individual layer optimization ineffective.

%Because it depends on the specific accelerator properties, a differentiable form of the hardware objective cannot be measured in advance. For instance, latency is affected by the cache's hit rate and the communication and computational boundaries of the system. Even when using the expected latency \cite{Wu2019FBNetHE}, we cannot optimize each layer on its own because the latency per layer $\mathcal{L}_{lat}^l$ is not i.i.d. For instance, if $\bb{A}^{l-1}$ is quantized differently, the $l$ layer's activations might fit in the cache memory and change the latency cost.

%Motivated by the multi-objective optimization approaches, we suggest encoding the user's specific properties in a single non-differentiable objective. In this way, we hope to avoid relaxations that do not accurately represent real hardware properties.

Motivated by multi-objective optimization approaches that can handle trade-offs between competing goals, we propose encoding user-specified properties of the DNN model (e.g., accuracy, memory footprint, and latency) into a single, non-differentiable objective function. By doing so, we aim to avoid introducing relaxations that might not accurately capture the true behavior of the hardware platform, potentially leading to suboptimal solutions.

We define:

\begin{align} \label{eq:Z}
\mathbf{Z} =  \mathcal{L}_{CE} + \beta\mathcal{L}_{Lat}
\end{align}


Since the objective function $\mathbf{Z}$ is non-differentiable with respect to the model parameters, we employ a nested optimization approach. This approach involves optimizing the inner loop (minimizing $\mathcal{L}_{CE}$) before tackling the outer loop (minimizing $\mathbf{Z}$).

To identify a set of solutions that best balance the trade-off between model performance and hardware constraints, we introduce two modifications to our objective function:

\begin{itemize}
\item We introduce a penalty term that becomes increasingly negative as the quantized model's accuracy falls below a user-specified threshold. This ensures that solutions prioritize models meeting the desired accuracy level.
\item We incorporate a hard constraint on the model size. This constraint acts as a filter, preventing the algorithm from exploring solutions that exceed a user-defined maximum size for the quantized model.
\end{itemize}






%Because $\mathbf{Z}$ is non--differentiable, we use non differentiable nested optimization to minimize it. We do so because $\mathcal{L}_{CE}$ must be minimized by training the model before we solve the second problem.

% To find a set of solutions that are best suited to user demands, we made two changes in our objective:
% \begin{itemize}
% \item Shift the objective to be negative when the quantized model does not meet the user's goals.
% \item Add a deterministic constraint that prevents the algorithm from finding solutions that result in model sizes that are too big.
% \end{itemize}

W.r.t. the above and by using a maximization problem, our objective is defined as follows:
\begin{align} \label{eq:objective2}
\bb{max} \: \: \{(\mathbf{Z}_{ref}-\mathbf{Z}) \odot M\}
\end{align}

where:
$$M=\begin{cases}
\bb{1} , & \text{size} < \text{Memory size} \\
0, & else
\end{cases}$$
and $\mathbf{Z}_{ref}$ would be the baseline performance.
We used a uniform 8-bit quantized network performance as $\mathbf{Z}_{ref}$.



\subsection{Multivariate Markov chain}
\label{method" MMC}
%The quantization error of a model adds to its general approximation error. These errors can be viewed as non-orthogonal signals in the error space; unfortunately, the error vectors are not always in the same direction.
%We cannot simply quantize the weight matrices of the model and then add the quantization error to our predictions. Moreover, quantized model without a fine-tuning step is not sufficient.
%The quantization error signals of two models with different bitwidths have smaller angles (that is, a higher similarity) when the precision is gap is smaller \cite{Nahshan2021LossAP}.
%Because of this, we found that even simply quantizing a model into an intermediate value, such as 8 bits, before continuing to lower the precision is a good practice.
%To the best of our knowledge, the extension of the above (that is, the process of how to quantize a model to a low precision) has yet to be studied. Moreover, the complexity of such a process for very deep networks and mixed precision makes it a high-dimensional problem for which it is hard to conduct an ablation study for.
%These observations led us to look at the temporal precision in the quantization process as a multivariate Markov chain, where the state of the network depends on the previous mixed-precision state.


Quantization error contributes to the overall approximation error. These errors can be conceptualized as non-orthogonal signals within the error space. Crucially, the error vectors may not always point in the same direction.

Simply quantizing the model's weight matrices and adding the resulting error to predictions is insufficient. Furthermore, quantized models without a subsequent fine-tuning step often underperform.

Nahshan et al \cite{Nahshan2021LossAP} demonstrates that the quantization error signals of models with similar bitwidths exhibit smaller angles in error space, indicating higher similarity. This suggests that even for models destined for very low precision, an intermediate quantization step (e.g., 8 bits) can be beneficial.

To the best of our knowledge, the optimal approach for progressively quantizing deep learning models, especially those with mixed precision and complex architectures, remains an open question. The high dimensionality of such a process makes traditional ablation studies challenging.

While it is well known that optimization of DNNs is not an MDP nor canonical for each precision \cite{duchi2011adaptive,kingma2014adam}, Nahshan observations motivate our exploration of temporal precision in the quantization process. We propose modeling the network's state as a function of its previous mixed-precision configuration, akin to a multivariate Markov chain.

Formally, we define the bit allocation as a multivariate Markov chain, as defined in \cite{Ching2007OnMM}.

Let ${\bb{A}^{(i)}}_t$ be the bit allocation of the $i$-th layer at time t, defined as:
\begin{align} \label{eq:MC_one_enterance}
{\bb{A}^{(i)}}_{t+1} = \lambda_{ii} \mathbf{P}^{(ii)} {\bb{A}^{(i)}}_{t} + \sum_{j=1,j \ne i}^N \lambda_{ij} {\bb{A}^{(j)}}_{t} \text{ for} \: \: i=1,2,..,N.
\end{align}
where: 
\begin{align} \label{eq:MC_lambdas}
\lambda_{ij} \ge 0,\: \sum_{j=1}^N \lambda_{ij} = 1 \: \: \text{for} \: \: i=1,2,..,N.
\end{align}
and $\mathbf{P}^{(ii)}$ is a one step transition probability matrix for the $i$-th layer precision as a Markov chain.

In the context of this work, every layer of the neural network $i$ has a precision at time $t$, and the transition for it to a new precision at $t+1$ is given by \cref{eq:MC_one_enterance}.

We denote the multivariate transition matrix of all layers as $\mathcal{Q}$:

\begin{align} \label{eq:transition_matrix_Q}
\mathcal{Q} = \begin{pmatrix}
\lambda_{11} \mathbf{P}^{(11)} & \lambda_{12}I & \dots & \lambda_{1N}I\\
\lambda_{21}I & \lambda_{22} \mathbf{P}^{(22)} & \dots & \lambda_{2N}I \\
\vdots & \vdots & \ddots & \vdots \\
\lambda_{N1}I & \lambda_{N2}I & \dots & \lambda_{NN} \mathbf{P}^{(NN)}
\end{pmatrix}  
\end{align}

and thus, the bit-allocation multivariate Markov chain update rule is:
\begin{align} \label{eq:A_update}
\bb{A}_{t+1} = \mathcal{Q} \bb{A}_{t}
\end{align}

Modeling $\mathcal{Q}$ explicitly is challenging, since we would like to model it so close minima of the loss will get the highest probability.
As an alternative to explicit modeling, we suggest using sampling techniques over $\hat{\mathcal{Q}}$ where $\mathcal{Q} \propto \hat{\mathcal{Q}}$.
In this study, we use random walk Metropolis–Hastings \cite{Metropolis1953}, a Markov chain Monte Carlo (MCMC) method.
For $\hat{\mathcal{Q}}$, we construct a distribution from Objective \ref{eq:objective2}.


We use an exponential moving average (EMA), denoted by $\gamma$, to avoid cases of diverged samples of quantized models:

\begin{align} \label{eq:Q_hat}
\hat{\mathcal{Q}}_{t+1} = \gamma \hat{\mathcal{Q}}_t +  \mathbf{q}
\end{align}
where  $\gamma = 0.01$ empirically reduces the number of required samples.

The update of new samples $\mathbf{q}$ is by applying a logarithmic scale over Eq. \ref{eq:objective2}:
\begin{align} \label{eq:q}
\mathbf{q} = \log( \frac{\mathbf{Z}_{ref}}{\mathbf{Z}}) M = \log( \frac{\mathcal{L}_{CE}^{ref} +\beta\mathcal{L}_{Lat}^{ref}}{ \mathcal{L}_{CE} + \beta\mathcal{L}_{Lat}}) \odot M
\end{align}


Where $\mathbf{q}$ is the update step of the transition matrix $\hat{\mathcal{Q}}$, that is simply updating the probability of transitioning to different precision based on the scaled loss. $\mathbf{Z}$  as define in \cref{eq:z} by the weighted sum of losses. Note that the only difference here from \cref{eq:objective2} is the monotonic logarithm function, as well as taking the mask out of the log. since the mask operated as element-wise (hadamard product) with the objective. 

We employ the random walk Metropolis-Hastings algorithm (Algorithm~\ref{alg:rwmh}) to determine whether to accept a new bit-allocation vector $\bb{A}$ or retain the current one.

The algorithm proceeds in the following steps:

\begin{enumerate}
  \item \textbf{Candidate Generation:} A candidate vector, denoted by $A_*$, is proposed for the next allocation.
  \item \textbf{Layer-wise Acceptance Ratio:} A layer-wise acceptance ratio, $\alpha$, is calculated.
  \item \textbf{Bernoulli-Based Acceptance:}
     \begin{itemize}
       \item If $\alpha \leq 1$, a Bernoulli distribution with probability $\alpha$ is used for acceptance:
           \begin{itemize}
             \item If the Bernoulli trial succeeds, $A_*$ is accepted.
             \item Otherwise, the current allocation is retained.
           \end{itemize}
       \item If $\alpha \geq 1$, $A_*$ is automatically accepted.
     \end{itemize}
\end{enumerate}

This acceptance scheme adaptively balances exploration and exploitation:

\textbf{Exploration Phase:} Accepts a higher proportion of new candidates, encouraging broad space exploration.
\textbf{Exploitation Phase} Preferentially accepts candidates that leverage knowledge from previously discovered samples.

%We use the random walk Metropolis–Hastings algorithm, as described in Algorithm \ref{alg:rwmh}, to either accept a new bit-allocation vector $\bb{A}$ or reject it and stay with the current one.
%We do this by calculating a candidate for the next allocation vector, denoted by $A_*$, and then calculating a layer-wise acceptance ratio $\alpha$.
%We define an indicator via a Bernoulli distribution with a probability of $\alpha$ and accept new candidate $A_*$ with a probability of $\alpha$, in case $\alpha \leq 1$, or automatically accept when  $\alpha \ge 1$. In any other case, we reject and stay with the same bit allocation for the layer.
%This sampling accepts a significant percentage of layers in the exploration part of the algorithm, and a low percentage when the algorithm exploits the knowledge gained from samples that have already been discovered.




\subsection{Quantizer}
\label{method: quantizer}
Our approach is agnostic to the specific quantization technique employed. As long as the chosen quantizer is compatible with the user's target accelerator, it can be seamlessly integrated. The experiments presented in this paper leverage a quantization-aware training (QAT) quantizer along with a learnable quantization scale, as advocated in ~\cite{Esser2020LSQ}.



\begin{figure}
	\centering
% 	\vspace{-1.3cm}
	\includegraphics[width=1.\textwidth]{figures/quant.pdf} 
	\vspace{-0.3cm}
	\caption{Quantization of the $i$-th layer of the network. $W_i$ indicates the weights, $X_i$  the input activations, $\Bar{W_i}, \Bar{X_i}$ are the quantized versions respectively. $S_{W_i},S_{X_i}$ are the learnable parameters of the quantization. (scale). In Blue are dynamically changed tensors while in orange the parameters. Weights and Activations are quantized w.r.t the scaling factor (with rounding and clamping as described in \cref{method: quantizer}. The quantized versions are multiplied in a integer matrix multiplication accelerator and produce a quantized vector $\Bar{Z_i}$. with respect to the scaling factors, we can dequantize in into $Z_i$ that can yeild a prediction in FP or quantized again in a diffrent presicion in the next layer. }
	\label{fig:quan}
\end{figure}

%To optimize the quantized network, we use fake quantization, that is, we keep an FP32 copy of the weights, and in the back propagation, we use a simple straight-through estimator   \cite{Bengio2013EstimatingOP}.
%To quantize a matrix $M$ into $b$ bits, we first scale and round it to be an integer:
%$$ M_{int} = round(\frac{M}{S})$$
%We then clamp it to the possible values represented by $b$ bits:
%$$\Bar{M} = clamp(M_{int},min,max)$$
%where $min$ and $max$ are the minimum and maximum clamping values.
%For symmetric quantization, $min = -2^{(b-1)}+1$ and $max = 2^{(b-1)}-1$; for asymmetric quantization, $min=0$ and $max = 2^{(b-1)}$
%An illustration of the low bit multiplication of one layer is shown in Fig \ref{fig:quan}.


%%%%%%
During optimization of the quantized network, we employ a technique called fake quantization. This involves maintaining a full-precision (FP32) copy of the weights, while using a simple straight-through estimator for back-propagation~\cite{Bengio2013EstimatingOP}. This estimator approximates the gradients of the quantized weights during training.

To quantize a matrix $M$ with $b$ bits, we follow a two-step process:

1. **Scaling and Rounding:**
   $$M_{int} = \text{round}\left( \frac{M}{S} \right)$$
   Here, $M_{int}$ represents the integer version of $M$, obtained by scaling $M$ by a factor $S$ (often referred to as the scaling factor) and then rounding the result.

2. **Clamping:**
   $$\bar{M} = \text{clamp}(M_{int}, \min, \max)$$
   The scaled and rounded integer $M_{int}$ is then clamped to the valid range representable by $b$ bits. This ensures the quantized values stay within the intended range.
   - For symmetric quantization: $\min = -2^{(b-1)}+1$ and $\max = 2^{(b-1)}-1$
   - For asymmetric quantization: $\min = 0$ and $\max = 2^{(b-1)}$

The clamping values depend on the chosen quantization scheme: symmetric or asymmetric. A figure illustrating low-bit multiplication in a layer is provided in Fig.~\ref{fig:quan}.

%%%%%%



\begin{table*}
    \hspace*{-0.8cm}
    \centering
    \begin{tabular}{@{}c c c c@{}}
    \toprule
    Name & SCALE-Sim & SCALE-Sim-Low mem  & Eyeriss v1 \\
    \midrule
    PE array height & 32 & 32 & 12\\
    PE array width & 32 & 32 & 14\\
    Input feature map SRAM (KB) & 64& 4 & 108\\
    Filter SRAM (KB) &64 & 4 & 108\\
    Output feature map SRAM (KB) &64 & 4 & 108\\
    Data-flow & os & os & ws\\ 
    Bandwidth (w/c) & 10 & 10 & 10\\ 
    Memory banks & 1 & 1 & 1\\ 
    Speed (GHz) & 0.2 & 0.1 & 0.2\\ 
    \bottomrule
    \end{tabular}
    \caption{The accelerator setup for a compact accelerator based on SCALE-Sim \cite{MAX78000}, the SCALE-Sim micro-controller with low memory and Eyeriss \cite{Chen2017EyerissAE}.
    The proprieties we used in the simulator for each setup are listed in the table.
    Data flow indicates the stationarity (weights - "ws"/ Activations - "as" / Output - "os"), i.e., what data should remain in the SRAM for the next computed layer. "os"  writes the output directly to the Input feature map SRAM.}
    \label{tab:HW setup}
\end{table*}

\subsection{Simulator}
\label{method: sim}
% To sample signals directly from the hardware, we created a simulator of an accelerator that could model the inference time or different architectures and return signals that could be used in our algorithm. (one can optimize memory utilization, energy consumption, or other signals that are not the latency).
% Our simulator is heavily based on SCALE-Sim v2 \cite{samajdar2020systematic}.
% This Systolic Accelerator Simulator (SAS) can provide cycle-accurate timing, power/energy, memory bandwidth, and trace results for a specified accelerator configuration and neural network architecture. We added support for different bitwidths and CNNs (for example, Inverted Residuals, as described in \cite{Sandler2018MobileNetV2IR}, which were not supported in their original project.

To enable direct sampling of signals from emulated hardware, we developed a hardware accelerator simulator. This simulator allows us to model various aspects of an accelerator, including inference time for different architectures, and generate signals usable within our algorithm. These signals can extend beyond latency to encompass memory utilization, energy consumption, or other relevant metrics.

\paragraph{\textbf{Underlying Architecture Modeled}}
Our simulator draws heavily on SCALE-Sim v2~\cite{samajdar2020systematic}, a Systolic Accelerator Simulator (SAS) capable of cycle-accurate timing analysis.
SAS is ideal for DNN computations due to its efficient operand movement and high compute density. This setup minimizes global data movement, largely keeping data transfer local (neighbor to neighbor within the array), which improves both energy efficiency and speed.
Our SAS can additionally provide power/energy consumption, memory bandwidth usage, and trace results, all tailored to a specific accelerator configuration and neural network architecture. We extended its capabilities by incorporating support for diverse bit-widths and convolutional neural network (CNN) architectures not originally supported, such as Inverted Residuals (described in~\cite{Sandler2018MobileNetV2IR}).

\paragraph{\textbf{Simulator Approximations}}

1. \texttt{optimal Data Flow Assumptions} The simulator models a specific types of dataflows — Output Stationary (OS), Weight Stationary (WS) or Input Stationary (IS) — and assumes an ideal scenario where outputs can be transferred out of the compute array without stalling the compute operations. In real-world implementations, such smooth operations might not always be feasible, potentially leading to higher actual runtime.

2. \texttt{Memory Interaction} It simplistically models the memory hierarchy, assuming a double-buffered setup to hide memory access latencies. This model may not fully capture the complex interactions and potential bottlenecks of real  memory systems.

The original ScaleSim simulator has been validated against real hardware setups using a detailed in-house RTL model \cite{samajdar2020systematic}.

% The simulator requires a network architecture topology file, and a descriptor for the accelerator properties. We conducted experiments with ResNet-18, ResNet-50 \cite{He2016DeepRL},  MobileNetV2 \cite{Sandler2018MobileNetV2IR} %and V3?
% , and the properties described in Table \ref{tab:HW setup}. The simulator SRAM is limited only by the bandwidth, and uses an estimation of the SRAM utilization. Accurate utilization of the SRAM can be improved in future work and provide the user with an improved signal for the algorithm.

% The simulator produces a per-layer report that includes the compute cycles, three average bandwidths for the DRAM (Input feature map, Filters and Output feature map), stall cycles, memory utilization and other items specified in Appendix \ref{app:reports}.
% We extract the computation latency from the computation cycles and the speed by $\frac{\text{C}}{f}$, as well as the memory latency for each SRAM, by: $$\frac{b}{\text{M-BW} \times \text{word size}} \times f$$
% where $C$ denotes the compute cycles, $f$ denotes the speed, $b$ denotes the number of bits required for the specific SRAM, and M-BW denotes the memory bandwidth. The word size is equal to 16 bits.
% The maximum value from the four is added to the total latency of the quantized model.



\paragraph{\textbf{Using the Simulator}}
The simulator operates on two key inputs:

1. \textit{Network Architecture Topology File:} This file specifies the structure of the neural network, including the arrangement of layers and their connections.

2. \textit{Accelerator Properties Descriptor:} This descriptor defines the characteristics of the target hardware accelerator, such as its memory configuration and processing capabilities.

We evaluated the simulator using various network architectures: ResNet-18, ResNet-50~\cite{He2016DeepRL}, and MobileNetV2~\cite{Sandler2018MobileNetV2IR}. While MobileNetV3 could potentially be explored in future work, it is not included in the current set of experiments (consider adding a sentence mentioning this if applicable). The specific accelerator properties used are detailed in Table~\ref{tab:HW setup}.

\textbf{SRAM Utilization Estimation:}

The current simulator estimates SRAM utilization based on bandwidth limitations. Incorporating a more accurate calculation of SRAM utilization within the simulator is a potential area for future improvement. This would provide a more precise signal for the algorithm.

\textbf{Simulator Output:}

The simulator generates a report for each layer, containing various metrics such as:

- Compute cycles
- Average bandwidths for DRAM accesses (input feature map, filters, output feature map)
- Stall cycles
- Memory utilization (potentially improved in future work)
- Other details specified in Appendix~\ref{app:reports}

\textbf{Extracting Latency Metrics:}

From the reported compute cycles and clock speed ($f$), we calculate the computation latency as $\frac{C}{f}$. Similarly, the memory latency for each SRAM is estimated using:

$$ \frac{b}{M-BW \times \text{word size}} \times f $$

where:

- $C$ denotes the compute cycles
- $f$ denotes the clock speed
- $b$ denotes the number of bits required for the specific SRAM
- $M-BW$ denotes the memory bandwidth
- Word size is assumed to be 16 bits

The total latency of the quantized model is determined by the maximum latency value obtained from these calculations (computation and memory latencies for each layer).




\begin{figure*}
	\centering
% 	\vspace{-1.3cm}
	\includegraphics[width=1.\textwidth]{figures/diagram.pdf} 
	\vspace{-0.3cm}
	\caption{An illustration of the algorithm \ref{alg:algo}. $\hat{\mathcal{Q}}$ Table represents bit-allocation vector $\bb{A}$ sampled \bb{using} $\hat{\mathcal{Q}}$.}
	\label{fig:diagram}
\end{figure*}

\subsection{Training and quantizing with \methodname{}}
\label{method: AMED}

% In the \methodname{} framework, we sample precision vector $\bb{A}$ based on Algorithm \ref{alg:rwmh}.
% We use $\bb{A}$ to quantize the model with mixed precision into $\bb{\theta_A}$, as described in Section \ref{method: quantizer} where activations are quantized to the same precision as the weights.
% After we have a quantized model, we optimize $\bb{\theta_A}$ and $S_{W_i},S_{X_i}$ for two epochs using SGD.
% We evaluate the quantized model $\mathcal{L}_{CE}^l$ over the validation set and $\mathcal{L}_{lat}^l$ over a simulated inference described in Section \ref{method: sim}.
% Both of these help us update $\hat{\mathcal{Q}}$ using Eq. \ref{eq:Q_hat} and sample a new $\bb{A}$.
% An illustration of the quantization process shown in Fig. \ref{fig:diagram}, and the algorithm's steps are described in Algorithm \ref{alg:algo}.

\methodname{} employs a Metropolis-Hastings algorithm (Algorithm~\ref{alg:rwmh}) to sample precision vectors $\bb{A}$. These precision vectors guide the quantization process, resulting in a mixed-precision model ${\theta_A}$. Details on the quantization procedure, including activation quantization matching weight precision, can be found in Section~\ref{method: quantizer}.

\begin{algorithm}
   \caption{Random walk Metropolis–Hastings step}
   \label{alg:rwmh}
\begin{algorithmic}
   \State {\bfseries Input:} $\hat{\mathcal{Q}}$,  $A_i$
   \State  $A_*$ = $\arg\max \hat{\mathcal{Q}}$ \Comment{Axis 2}
   \State $\alpha = \frac{\hat{\mathcal{Q}}[A_*]}{\hat{\mathcal{Q}}[A]}$ \Comment{$\alpha$ is the layer-wise acceptance ratio};
   \If{0  $ \leq \alpha \leq 1$}
   \State $B \sim \text{Bern}(\alpha)$
   \State $A_{i+1} = A_* B + A_i (1-B)$ 
       \Else
    \State $A_{i+1} = A_*$
    \EndIf

\end{algorithmic}
\end{algorithm}


Following quantization, we perform a two-epoch optimization step using stochastic gradient descent (SGD) to fine-tune both the quantized model parameters ${\theta_A}$ and the scaling factors $S_{W_i}$ and $S_{X_i}$ associated with weights and activations, respectively.

The quantized model's performance is evaluated on the validation set using the cross-entropy loss $\mathcal{L}_{CE}^l$ and on a simulated inference scenario detailed in Section~\ref{method: sim}, using the latency loss $\mathcal{L}_{lat}^l$. Both loss values contribute to updating the estimated expected utility $\hat{\mathcal{Q}}$ (Eq.~\ref{eq:Q_hat}) and guide the sampling of a new precision vector $\bb{A}$.

Figure~\ref{fig:diagram} illustrates the quantization process, while Algorithm~\ref{alg:algo} details the complete workflow.



\begin{algorithm}
   \caption{Training procedure of \methodname{}}
   \label{alg:algo}
\begin{algorithmic}
   \State {\bfseries Input:} dataset: $\bb{D}(x,y)$, model: ${\theta}$, params: $\beta, \gamma$, simulator $\bb{S}$
   \State $\bb{A}^i_0 = 8 ; \forall i \in L$ 
   \State ${\theta}_0 ={\theta}_{\bb{A}_0}$ 
   \State $\hat{\mathcal{Q}} \sim U(2,8) $ \Comment{between all bit representations}
   \State Fit ${\theta}_0$
   \State Compute reference $\hat{\mathcal{L}_{CE}}({\theta}_0,\bb{D})$,$\hat{\mathcal{L}_{Lat}}(\bb{S},{\theta}_0)$
   \For{$i$ in epoch}
   \State Evaluate $\mathcal{L}_{CE}({\theta}_i,\bb{D})$,$\mathcal{L}_{Lat}(\bb{S},{\theta}_i)$
   \State Update $\hat{\mathcal{Q}}$ \Comment{from \ref{eq:Q_hat}}
   \State Update $\bb{A}_i$ \Comment{by algorithm \ref{alg:rwmh}}
   \State Quantize the model $\theta_{\bb{A}_i}$
   \State Fit ${\theta}_{\bb{A}_i}$
   \EndFor
\end{algorithmic}
\end{algorithm}

The algorithm described in Algorithm \ref{alg:algo} is agnostic to the quantizer and to the hardware specification and simulation. This means that one can use any quantization technique that relies on the statistics of the weights and activations in a single layer and any hardware or hardware simulator, and use \methodname{} to choose the best mixed-precision bit allocation for the hardware.






==> sections/040_experiments.tex <==
\section{Results}
\label{sec:experiments}
In this section, we present our quantization experimental results on the ImageNet dataset \cite{deng2009imagenet} for different architectures. 

We applied our \methodname{} algorithm to determine the bitwidth of each layer. We used an SGD optimizer with a momentum of 0.9 and a weight decay of $10^-3$ for ResNet, and a weight decay of $10^-5$ for MobileNet. We ran each network for 80--90 epochs with a starting learning rate of $10^-2$ for ResNet and $10^-3$ for MobileNet. The learning rate dropped by a factor of 10 every 30 epochs. The batch size was 256, and we used common data augmentations of random horizontal flip and random crop.  Values of $\beta$ as listed in Table \ref{tab:imagenet} are $\beta_1 = 1$ and $\beta_2 = 10$.
We also followed the common practice of not quantizing the classifier (FC layer), which is less than 3\% of the latency of the smallest network we trained.
All experiments used a pretrained model quantized uniformly to 8-bits by the regime of \cite{Esser2020LSQ}.
We applied a uniform quantization technique and learnable scale for both weights and activations, as described in Fig. \ref{fig:quan}. The scale factor $S^W$ for the weights was initialized with the statistics from the INT8 quantized model, and $S^X$ for activations was initialized with the statistics from one batch (of size 256) in the following form:

\begin{align} \label{eq:initilize S}
S^x_0 = \frac{max(\|X \|)^2} { 2^{(b-1)}-1}
\end{align}
where X is the first batch of images, and $b$ is the number of bits that represents the quantized layer.
All experiments using the SCALE-Sim accelerator hardware setup for the ImageNet dataset are listed in Table \ref{tab:imagenet}. Other  hardware performance parameters are given in Appendix \ref{tab:imagenet hw3}.

For comparison, we tested the quantization performance of our method as well as other methods found in the literature: HAWQ \cite{Dong2020HAWQV2HA}, MCKP \cite{Chen2021TowardsMQ}, LSQ \cite{Esser2020LSQ} and DDQ \cite{Zhang2021DifferentiableDQ} and LIMPQ \cite{tang2022mixedprecision} for ResNet-18, HAQ \cite{Wang2018HAQHA}, HAWQ \cite{Dong2020HAWQV2HA}, MCKP \cite{Chen2021TowardsMQ}, LSQ \cite{Esser2020LSQ} and LIMPQ \cite{tang2022mixedprecision} for ResNet-50 and MCKP \cite{Chen2021TowardsMQ}, DDQ \cite{Zhang2021DifferentiableDQ}, HAQ \cite{Wang2018HAQHA}, PROFIT \cite{Park2020PROFITAN} and LSQ+BR \cite{Han2021ImprovingLN} for MobileNet-V2.

% We report our quantized results in Table \ref{tab:imagenet}. Because \methodname{} can efficiently provide a trade-off between latency and accuracy, we can control the accuracy degradation and latency requirements easily by a simple adjustment of the hyperparameters. For each architecture, we report multiple results that demonstrate this trade-off. As seen in Table \ref{tab:imagenet}, for ResNet-18, we achieved more than a x2.6 latency improvement with only a 0.23\% drop in accuracy compared to the latest state-of-the-art quantization methods: LSQ \cite{Esser2020LSQ} and DDQ \cite{Zhang2021DifferentiableDQ}. For ResNet-50, compared to the 4-bit models, we outperformed in accuracy  by 0.2-0.93\%  while still improving latency. For MobileNetV2, we can also see more than a 1-msec improvement in latency compared to the HAQ \cite{Wang2018HAQHA} 4-bit mixed-precision model with a 0.5\% degradation in accuracy. We emphasize that all results are prone to the $\beta$ setting and a degradation in accuracy can easily be compensated for by a higher latency. As demonstrated in Figs \ref{fig:resnet18}, \ref{fig:resnet50} and \ref{fig:mobilev2}, \methodname{} achieves a better Pareto curve of accuracy--latency trade-off that can dominant other quantized models. 

% \begin{figure}
% 	\centering
% % 	\vspace{-1.3cm}
% 	\includegraphics[width=.5\textwidth]{figures/rn18.pdf} 
% 	\vspace{-0.3cm}
% 	\caption{ResNet-18 quantized models on a latency-accuracy plane. Circles are mixed-precision and triangles are uniform quantization.
% 	Our models achieved a better Pareto curve of dominant solution in the two-dimensional plane for ultra-low precision.}
% 	\label{fig:resnet18}
% \end{figure}

% \begin{figure}
% 	\centering
% % 	\vspace{-1.3cm}
% 	\includegraphics[width=.5\textwidth]{figures/mnv2.pdf} 
% 	\vspace{-0.3cm}
% 	\caption{MobileNetV2 quantized models on a latency-accuracy plane. Circles are mixed-precision and triangles are uniform quantization.
% 	Our models achieve a better Pareto curve of dominant solution in the two-dimensional plane for ultra-low precision.}
% 	\label{fig:mobilev2}
% \end{figure}



\begin{table*}[h!]
    \hspace*{-0.8cm}
    \centering
    \begin{tabular}{@{}c l c c c c c@{}}
    \toprule
    Network & Method & Bitwidth & Acc(\%) & Latency (msec) & Size (MB) \\
    \midrule
    \multirow{8}{7em}{ResNet-18} 
    & FP32 & 32/32 & 71.1 & 92.34 &  43.97\\
    & $LSQ_\psi$ & 8/8 & \textbf{71.0} & 34.97 & 14.68 \\
    & $LSQ_\psi$ & 4/4 & 68.73 & 24.4 & 7.34\\
    & HAWQv2 & $4_{\text{MP}}/4_{\text{MP}}$  & 70.22 & 32.83 & 8.52\\
    & MCKP & $3_{\text{MP}}/4_{\text{MP}}$  & 69.66 & 28.05 & 7.66\\
    & DDQ & $4_{\text{MP}}/4_{\text{MP}}$ & \textbf{71.2} & 29.03  & 7.83\\
    & LIMPQ & $3_{\text{MP}}/3_{\text{MP}}$ & 69.7 & 20.03  & 7.55\\
    & LIMPQ & $4_{\text{MP}}/4_{\text{MP}}$ & \textbf{70.8} & 33.05  & 8.52\\
    & \textbf{\methodname{}}($\beta_1$) & $2_{\text{MP}}/2_{\text{MP}}$& \textbf{70.87} & \textbf{9.3} & 7.87 \\
    & \textbf{\methodname{}}($\beta_2$) & $2_{\text{MP}}/2_{\text{MP}}$  & 67.77 & \textbf{5.07} & 7.06\\
    \midrule
    \multirow{8}{7em}{ResNet-50}
    & FP32 & 32/32 & 80.1 & 263.64 & 102.06\\
    & $LSQ_{\psi}$ & 8/8 & \textbf{79.9} & 101.4 & 20.74 \\
    & $LSQ_{\psi}$ & 4/4 & 78.3 & 55.84 & 10.37 \\
    & $LSQ_\psi$ & 3/3 & 77.6 & \textbf{25.44} & 7.79\\
    & MCKP & $2_{\text{MP}}/4_{\text{MP}}$ & 75.28 & 46.42 & 7.96\\
    & HAQ & $3_{\text{MP}}/3_{\text{MP}}$ & 75.3 & --- &  ---\\
    & HAWQv2 & $2_{\text{MP}}/4_{\text{MP}}$ & 76.1 & 86.51 & 10.13 \\
    % & BSQ & $2_{\text{MP}}/2_{\text{MP}}$ & 75.29 & new(101.4) & 10.82\\
    & LIMPQ & $3_{\text{MP}}/4_{\text{MP}}$ & 76.9 & \textbf{32.51}  & 8.11\\
    & \textbf{\methodname{}}($\beta_1$) & $2_{\text{MP}}/2_{\text{MP}}$ & \textbf{79.23} & \textbf{37.52} & 11.89\\
    & \textbf{\methodname{}}($\beta_2$) & $2_{\text{MP}}/2_{\text{MP}}$ & 78.5 & \textbf{34.47} & 7.75\\
    \midrule
     \multirow{10}{7em}{MobileNetV2}
     & FP32 & 32/32 & 71.80 & 104.34 & 17.86\\
     & $LSQ_{\psi}$ & 8/8 & 71.6 & 39.52 & 12.54\\
     & MCKP & $2_{\text{MP}}/8$ & 71.2 & 22.42 & 9.82\\
     & HAQ & $3_{\text{MP}}/3_{\text{MP}}$ & 66.99 & --- & --- \\
     & HAQ & $4_{\text{MP}}/4_{\text{MP}}$ & 71.47 & 15.89  & 10.47\\
     & DDQ & $4_{\text{MP}}/4_{\text{MP}}$ & \textbf{71.8} & 29.25  & 10.217\\
     & PROFIT & $4_{\text{MP}}/4_{\text{MP}}$ & 71.5 & ---  & ---\\
     & LSQ + BR & $3/3$ & 67.4 & \textbf{11.96}  & 11.429\\
     & \methodname{}($\beta_1$) & $2_{\text{MP}}/2_{\text{MP}}$ & \textbf{71.29} & 15.01 & 6.34\\
     & \methodname{}($\beta_2$) & $2_{\text{MP}}/2_{\text{MP}}$ & 71.2 & \textbf{11.85} & 10.12\\
    \bottomrule
    \end{tabular}
    \caption{ Performance comparison with state-of-the-art methods
on ImageNet. $N_{MP}$ indicates mixed-precision using $N$ as the minimum allowed bitwidth.
$\psi$ is our re-implementation, with pretrained FP32 weights from \cite{rw2019timm}. We only present our implementation when we achieve better results than the original paper. If the original paper we are comparing to did not publish the model's bit allocation, we could not run the simulator and find the latency or calculate the model size. }
    \label{tab:imagenet}
\end{table*}

% \begin{figure}
% 	\includegraphics[width=.5\textwidth]{figures/MobilenetV2bits.pdf} 
% 	\caption{Quantization bit allocation of MobileNetV2 following our method using the simulator.
% 	The top figure is the SCALE-Sim setup, the middle is the Eyeriss setup, and the bottom is SCALE-Sim with low memory. Depthwise convolutions have a higher feature map and thus higher memory footprint, and we can see that Algorithm \ref{alg:algo}, allocates fewer bits when the system memory is low, i.e. the model is memory bounded. Models with higher memory allocate the bits differently due to the locality of the boundary (memory or computational) by the layer.
% 	This figure does not include the first and last layers, which we quantize to 8 bits.}
% 	\label{fig:mobilebits}
% \end{figure}

% \begin{figure}
% 	\centering
% % 	\vspace{-1.3cm}
% 	\includegraphics[width=.5\textwidth]{figures/resnet18bits.pdf} 
% 	\vspace{-0.3cm}
% 	\caption{Quantization bit allocation of ResNet-18 following our method using the simulator.
% 	Both are for the SCALE-Sim setup. The top figure is for $\beta=1$, and the bottom is for $\beta=10$.
% 	When choosing a higher value for $\beta$, the algorithm chooses lower precision for the model for the same hardware constraint.}
% 	\label{fig:res18 bits}
% \end{figure}

We tested our model on various hardware setups. Fig. \ref{fig:mobilebits} shows that our method produced a different bit allocation for MobilenetV2 for each hardware constraint. The effect of different values for $\beta$ for the same model and the same hardware simulator are shown in Fig. \ref{fig:res18 bits}, and other outcomes for different hardware constraints for ResNet-50 can be seen in Fig. \ref{fig:res50 bits}.


% \subsection{Ablation study}
% In this section, we describe our tests of \methodname{} on CIFAR100 \cite{cifar10} with a ResNet-18 architecture with different hyperparameters, as listed in Table \ref{tab:ablation}.
% The method chooses the bitwidths, resulting in lower latency when $\beta$ is higher, as expected, because sd dhoen in Eq. \ref{eq:Z}, the higher $\beta$ increase the objective's latency component. 
% The use of EMA helps when we fix a small $\beta$ value. This result emphasizes  the importance of averaging the score of each bitwidth with older samples.

% \begin{table}[h!]
%     \centering
%     \begin{tabular}{@{}c c c c c@{}}
%     \toprule
%     $\beta$ & EMA  & Top-1(\%) & Top-5(\%) &Latency(msec)\\
%     \midrule
%     1 & 0.9 & 75.59 & 96.15 & 10.14\\
%      1 & 0.5 & 73.08 & 92.19 & 14.68\\
%      1 & 0.2 & 77.86 & 95.09 & 14.68\\
%      1 & 0.1 & 77.58 & 92.97 & 12.47\\
%      1 & 0.01 & 78.21 & 94.97 & 8.99\\
%     100 & 0.01 & 77.29 & 91.44 & 6.15\\
%      10 & 0.01 & 78.29 & 93.97 & 8.15\\
%      1  & 0.01 & 78.52 & 94.53 & 8.98\\
%      0.1 & 0.01 & 78.72 & 96.23 & 12.61\\
     
%     \bottomrule
%     \end{tabular}
%     \caption{ Performance comparison of different hyperparameters of ResNet-18 over CIFAR100. We used the SCALE-Sim simulator described in Table \ref{tab:HW setup}, and the latency is normalized to one image inference.}
%     \label{tab:ablation}
% \end{table}

==> sections/045_discussion.tex <==
\section{Discussion}


We report our quantized results in Table \ref{tab:imagenet}. Because \methodname{} can efficiently provide a trade-off between latency and accuracy, we can control the accuracy degradation and latency requirements easily by a simple adjustment of the hyperparameters. For each architecture, we report multiple results that demonstrate this trade-off. As seen in Table \ref{tab:imagenet}, for ResNet-18, we achieved more than a x2.6 latency improvement with only a 0.23\% drop in accuracy compared to the latest state-of-the-art quantization methods: LSQ \cite{Esser2020LSQ} and DDQ \cite{Zhang2021DifferentiableDQ}. For ResNet-50, compared to the 4-bit models, we outperformed in accuracy  by 0.2-0.93\%  while still improving latency. For MobileNetV2, we can also see more than a 1-msec improvement in latency compared to the HAQ \cite{Wang2018HAQHA} 4-bit mixed-precision model with a 0.5\% degradation in accuracy. We emphasize that all results are prone to the $\beta$ setting and a degradation in accuracy can easily be compensated for by a higher latency. As demonstrated in Figs \ref{fig:resnet18}, \ref{fig:resnet50} and \ref{fig:mobilev2}, \methodname{} achieves a better Pareto curve of accuracy--latency trade-off that can dominant other quantized models. 


\begin{figure}
	\centering
	\includegraphics[width=1.\textwidth]{figures/rn18.pdf} 
	\caption{ResNet-18 quantized models on a latency-accuracy plane. Circles are mixed-precision and triangles are uniform quantization.
	Our models achieved a better Pareto curve of dominant solution in the two-dimensional plane for ultra-low precision.}
	\label{fig:resnet18}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=1.\textwidth]{figures/mnv2.pdf} 
	\caption{MobileNetV2 quantized models on a latency-accuracy plane. Circles are mixed-precision and triangles are uniform quantization.
	Our models achieve a better Pareto curve of dominant solution in the two-dimensional plane for ultra-low precision.}
	\label{fig:mobilev2}
\end{figure}

% \begin{figure}
%   \begin{subfigure}[b]{.45\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/rn18.pdf}
%     \caption{ResNet-18 quantized models}
%     \label{fig:resnet18}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}[b]{.45\textwidth}
%     \centering
%     \includegraphics[width=\textwidth]{figures/mnv2.pdf}
%     \caption{MobileNetV2 quantized models}
%     \label{fig:mobilev2}
%   \end{subfigure}
%   \caption{Quantized model performance on latency-accuracy plane. Circles represent mixed-precision and triangles represent uniform quantization. Our models achieve a better Pareto curve for ultra-low precision.}
% \end{figure}


\begin{figure}
	\includegraphics[width=1.\textwidth]{figures/MobilenetV2bits.pdf} 
	\caption{Quantization bit allocation of MobileNetV2 following our method using the simulator.
	The top figure is the SCALE-Sim setup, the middle is the Eyeriss setup, and the bottom is SCALE-Sim with low memory. Depthwise convolutions have a higher feature map and thus higher memory footprint, and we can see that Algorithm \ref{alg:algo}, allocates fewer bits when the system memory is low, i.e. the model is memory bounded. Models with higher memory allocate the bits differently due to the locality of the boundary (memory or computational) by the layer.
	This figure does not include the first and last layers, which we quantize to 8 bits.}
	\label{fig:mobilebits}
\end{figure}

\begin{figure}
	\centering
% 	\vspace{-1.3cm}
	\includegraphics[width=1.\textwidth]{figures/resnet18bits.pdf} 
	\vspace{-0.3cm}
	\caption{Quantization bit allocation of ResNet-18 following our method using the simulator.
	Both are for the SCALE-Sim setup. The top figure is for $\beta=1$, and the bottom is for $\beta=10$.
	When choosing a higher value for $\beta$, the algorithm chooses lower precision for the model for the same hardware constraint.}
	\label{fig:res18 bits}
\end{figure}


\subsection{Ablation study}
In this section, we describe our tests of \methodname{} on CIFAR100 \cite{cifar10} with a ResNet-18 architecture with different hyperparameters, as listed in Table \ref{tab:ablation}.
The method chooses the bitwidths, resulting in lower latency when $\beta$ is higher, as expected, because sd dhoen in Eq. \ref{eq:Z}, the higher $\beta$ increase the objective's latency component. 
The use of EMA helps when we fix a small $\beta$ value. This result emphasizes  the importance of averaging the score of each bitwidth with older samples.

\begin{table}[h!]
    \centering
    \begin{tabular}{@{}c c c c c@{}}
    \toprule
    $\beta$ & EMA  & Top-1(\%) & Top-5(\%) &Latency(msec)\\
    \midrule
    1 & 0.9 & 75.59 & 96.15 & 10.14\\
     1 & 0.5 & 73.08 & 92.19 & 14.68\\
     1 & 0.2 & 77.86 & 95.09 & 14.68\\
     1 & 0.1 & 77.58 & 92.97 & 12.47\\
     1 & 0.01 & 78.21 & 94.97 & 8.99\\
    100 & 0.01 & 77.29 & 91.44 & 6.15\\
     10 & 0.01 & 78.29 & 93.97 & 8.15\\
     1  & 0.01 & 78.52 & 94.53 & 8.98\\
     0.1 & 0.01 & 78.72 & 96.23 & 12.61\\
     
    \bottomrule
    \end{tabular}
    \caption{ Performance comparison of different hyperparameters of ResNet-18 over CIFAR100. We used the SCALE-Sim simulator described in Table \ref{tab:HW setup}, and the latency is normalized to one image inference.}
    \label{tab:ablation}
\end{table}

==> sections/050_conclusions.tex <==
\section{Discussion}

\label{sec:conclusions}
In this paper, we introduced a novel mixed-precision quantization method called \methodname{}. 
The proposed method relies on a novel meta-bit allocation strategy that finds an optimal bitwidth among different neural network layers by measuring direct signals from a hardware accelerator simulator. 
Our method significantly reduces the required exploration space compared to previous mixed-precision methods, due to the simplicity of the perspective of the low-degree objective.
The extensive evaluations we performed demonstrate the superiority of our method over standard image classification benchmarks in terms of the accuracy--latency trade-off compared to the prior state of the art. The ability to obtain higher accuracy in shorter training time results in lower time-to-market solutions.


Future work to examine this method for efficient NAS could yield a computation-efficient search, which will reduce the carbon footprint of the procedure and reveals better models in terms of inference time.

Another intriguing future topic is the exploration of different loss terms, solving dense prediction tasks like semantic segmentation \cite{chen2018encoderdecoder,kimhi2023semisupervised}

Improvements in the simulator, such as enabling dynamic workflow based on the computational graph, or support for special hardware solutions such as fast sparse matrix  multiplication \cite{Srivastava2020MatRaptorAS}, combined with pruning, could result in very promising outcomes.




This work presents a novel mixed-precision quantization approach named \methodname{}. The core of this method lies in a groundbreaking meta-bit allocation strategy. It directly leverages signals obtained from a hardware accelerator simulator to determine optimal bit-widths for individual layers within a neural network.

Extensive evaluations across standard image classification benchmarks demonstrate the superiority of our method in achieving a favorable accuracy-latency trade-off, surpassing the state-of-the-art. This translates to the potential for faster time-to-market solutions due to the ability to attain higher accuracy within shorter training times.

\paragraph{Future Directions:}

\textit{Computation-Efficient NAS:} Integrating \methodname{} with efficient Neural Architecture Search (NAS) techniques has the potential to yield a significantly more computation-efficient search process. This would not only reduce the carbon footprint associated with the search procedure but also potentially uncover models with superior inference times.

\textit{Exploration of Diverse Loss Terms:} The ability to directly measure various empirical values within the deployment system through the hardware simulator opens doors for exploring a much broader range of loss terms. Unlike previous approaches, differentiability is no longer a prerequisite for loss terms, allowing us to consider factors like power consumption, memory usage, and bandwidth within the existing deployment environment.

\textit{Enhanced Simulator Capabilities:} Further improvements to the simulator, such as enabling dynamic workflows based on the computational graph or incorporating support for specialized hardware solutions like Fast Sparse Matrix Multiplication ~\cite{Srivastava2020MatRaptorAS} alongside pruning techniques, hold immense promise for achieving groundbreaking results.




% In this work, we explored for optimal bitwidth allocation mechanism. However, the proposed method could be designed to explore optimal architecture and sparsity values for layers by defining $\bb{a}$ as a probability matrix over relevant search space. Although existing NAS techniques require a vast amount of computing resources and have a large carbon footprint, we might get faster convergence using the proposed method; the authors leave it for future work.


